Congested Urban Networks Tend to Be Insensitive to Signal Settings: Implications for Learning-Based Control

This paper highlights several properties of large urban networks that can have an impact on machine learning methods applied to traffic signal control. In particular, we show that the average network flow tends to be independent of the signal control policy as density increases. This property, which so far has remained under the radar, implies that deep reinforcement learning (DRL) methods becomes ineffective when trained under congested conditions, and might explain DRL's limited success for traffic signal control. Our results apply to all possible grid networks thanks to a parametrization based on two network parameters: the ratio of the expected distance between consecutive traffic lights to the expected green time, and the turning probability at intersections. Networks with different parameters exhibit very different responses to traffic signal control. Notably, we found that no control (i.e. random policy) can be an effective control strategy for a surprisingly large family of networks. The impact of the turning probability turned out to be very significant both for baseline and for DRL policies. It also explains the loss of symmetry observed for these policies, which is not captured by existing theories that rely on corridor approximations without turns. Our findings also suggest that supervised learning methods have enormous potential as they require very little examples to produce excellent policies.

==> pream.tex <==
\oddsidemargin 0.0in
\topmargin -0.5in
\headheight 0.3in
\headsep 0.2in
\textwidth 6.5in
\textheight 9.0in
\setlength{\parindent}{0.5in}

% PAGE HEADER
%------------------------------------------
% Adjust the header text below (INSERT AUTHORS HERE)
\oddsidemargin 0.0in
\usepackage[tiny,rm]{titlesec}

\newpagestyle{trbstyle}{
\sethead{Laval, and Zhou}{}{\thepage}% Change to the last names of the authors, use et al. if 4+ authors
}
\pagestyle{trbstyle}

% HEADINGS
%------------------------------------------
\renewcommand*{\refname}{\uppercase{References}}
\titleformat{\section}{\bfseries}{}{0pt}{\uppercase}
\titlespacing*{\section}{0pt}{12pt}{*0}
\titleformat{\subsection}{\bfseries}{}{0pt}{}
\titlespacing*{\subsection}{0pt}{12pt}{*0}
\titleformat{\subsubsection}{\itshape}{}{0pt}{}
\titlespacing*{\subsubsection}{0pt}{12pt}{*0}

% LISTS
%------------------------------------------
% Adjust lists a little. Not quite perfectly fitting TRB style, but vaguely
% close at least.
\usepackage[inline]{enumitem}
\setlist[1]{labelindent=0.5in,leftmargin=*}
\setlist[2]{labelindent=0in,leftmargin=*}

% CAPTIONS
%------------------------------------------
% Get the captions right. Authors must still be careful to use "Title Case"
% for table captions, and "Sentence case." for figure captions.
\usepackage{ccaption}
\usepackage{amsmath}
\usepackage{empheq}
\usepackage{multirow}
\usepackage{amssymb}
\makeatletter
\renewcommand{\fnum@figure}{\textbf{FIGURE~\thefigure} }
\renewcommand{\fnum@table}{\textbf{TABLE~\thetable} }
\makeatother
\captiontitlefont{\bfseries \boldmath}
\captiondelim{\;}
%\precaption{\boldmath}



% FONTS
%------------------------------------------
% Times for text and math
\usepackage{mathptmx}

% Some pdf conversion tricks? Unsure.
\usepackage[T1]{fontenc}
\usepackage{textcomp}
% Fonts will be broken by Sweave without this option


% CITATIONS
%------------------------------------------
% TRB uses an Author (num) citation style. I haven't found a way to make
% LaTeX/Bibtex do this automatically using the standard \cite macro, but
% this modified \trbcite macro does the trick.

% TODO: sort&compress option?
\usepackage[sort,numbers]{natbib}
\newcommand{\trbcite}[1]{\citeauthor{#1} ({\it \citenum{#1}})}
\setcitestyle{round}

% Reduce spacing between bibliographic items
\setlength{\bibsep}{0pt plus 0.3ex}


% LINE NUMBERING
%------------------------------------------
% TRB likes line numbers on drafts to help reviewers refer to parts of the
% document. Comment out for final versions.

% Use this for draft submissions - line numbering... sort of.
%\usepackage{parano}
%\renewcommand\theparano{\textbf{\scriptsize [\arabic{parano}]}}
% Use this for final submissions - no line numbering
%\newcommand{\parano}{}

% Add line numbers
\usepackage[pagewise]{lineno}
  \renewcommand\linenumberfont{\normalfont\small}


% COUNTERS
%------------------------------------------
% TRB requires the total number of words, figures, and tables to be displayed on
% the title page. This is possible under the totcount and the xparse packages on CTAN.
%
% Note that a total word count is added in V 2.1 to print a single value that is 
% calculated as: numberofwords + numberoffigures*250 + numberoftable*250

\newread\somefile
\usepackage{xparse}



\newcounter{totalwordcounter}
\newcounter{wordcounter}
\makeatletter

\NewDocumentCommand{\wordcount}{s}{%
  \immediate\write18{texcount -sum -1 \jobname.tex > count.txt}%
  \immediate\openin\somefile=count.txt%
  \read\somefile to \@@localdummy%
  \immediate\closein\somefile%
  \setcounter{wordcounter}{\@@localdummy}%
  \IfBooleanF{#1}{%
  \@@localdummy%   print only if not starred version
  }%
}
\makeatother
\usepackage{totcount}
	\regtotcounter{table} 	%count tables
	\regtotcounter{figure} 	%count figures

\newcommand{\wordfigure}{250} % number of words per figure
\newcommand{\wordtable}{250} % number of words per table

\newcommand{\totalwordcount}{%
  \wordcount*% The star allows just getting the number, not printing it
  \setcounter{totalwordcounter}{\value{wordcounter}}%
  %\addtocounter{totalwordcounter}{\numexpr\wordfigure*\totvalue{figure}}%
  \addtocounter{totalwordcounter}{\numexpr\wordtable*\totvalue{table}} % 
  \number\value{totalwordcounter}% Output the number
  \renewcommand{\totalwordcount}{\number\value{totalwordcounter}}% Prevent the call again, otherwise the figure/table counter would be added again. 
}



% OTHER PACKAGES
%------------------------------------------
% Add any additional \usepackage declarations here.

\usepackage{graphicx}


% TITLEPAGE
%-----------------------------------------


==> recycle.tex <==
In \cite{chin2012q}, the authors defined four levels of congestion based on the queue length at an intersection with four signal phases, thus the state space has a size of $2^4*2^4=256$. The action list is consisted of 1s to 5s of green time distribution.   



The value function is the
expected infinite discounted sum of reward that the agent will gain if
it starts in that state and executes the optimal policy  $\pi$.
%\[V^*(s) = \max_\pi E\left(\sum_{t=0}^\infty \gamma^t r_t\right)\;\;.\]
This optimal value function is unique and can be defined as the
solution to the Bellman equation:
\begin{equation}
V(s) = \max_a\left(R(s,a) + \gamma \sum_{s' \in {\cal S}}
                        P(s,a,s')V(s')\right), \forall s \in {\cal S}\;\;,
\label{e:vstar}
\end{equation}  
which assert that the value of a state $s$ is the expected
instantaneous reward plus the expected discounted value of the next
state, using the best available action.
Given the optimal value function, we can specify the optimal policy as
\begin{equation}
\pi(s) = {\rm arg} \max_a\left(R(s,a) + \gamma \sum_{s' \in {\cal
S}}P(s,a,s')V(s')\right) \;\;.
\label{e:pi}
\end{equation}  

Q-learning 88ref 
is a very popular method   based on approximations of the value-action function. For a given policy \( \pi  \),
we define the {state-action value} as \[
Q_{\pi }(s,a)\equiv (1-\gamma ){R}(s,a)+\gamma E_{s^{\prime };s,a)}\left[ V_{\pi }(s^{\prime })\right] \]




Here we consider dynamic demand profiles to see how the demand rate of change affects the learning framework.

We start with the case of a linearly increasing demand:  starting with an empty network, the network density increases linearly until reaching $k=1$ over a period of $T$ time steps of the learning framework, or equivalently $gT$ time steps of the CA model. This gives a demand rate of change of:
\begin{equation}\label{rate}
    \phi=1/(gT)
\end{equation}
in dimensionless form, or $\phi=\kappa^2 w/(gT)$ in real coordinates.




@ARTICLE{Ma2016Method,
timestamp={2017.05.29},
cat= {\textit{Category: }\textbf{PEDESTRIAN}},
author={Ma, J.a  and Xu, S.a  and Fan, W.a  and Song, W.b },
title={Method of bottleneck identification for massive crowd circulating network},
journal={Xitong Gongcheng Lilun yu Shijian/System Engineering Theory and Practice},
year={2016},
volume={36},
number={1},
pages={164-173},
doi={10.12011/1000-6788(2016)01-0164-10},
noteD={\textbf{Cited by 0, No PDF Available}},
url2={https://goo.gl/Ocyl8Y},
affiliation={National United Engineering Laboratory of Integrated and Intelligent Transportation, School of Transportation and Logistics, Southwest Jiaotong University, Chengdu, China; State Key Laboratory of Fire Science, University of Science and Technology of China, Hefei, China},
abstract={\textit{Abstract: }Under scenario of sports events and other kinds of massive gathering, a large amount of people would travel along road networks, thus forming crowded pedestrians. The high density situation might induce in mass panic and stampede, causing serious injuries and casualties. Therefore, it is necessary to firstly understand pedestrian flow features on the corresponding network and then apply proper control method to organize and manage pedestrian flow. Firstly, considering general characteristics of travelers' route choice behavior, all these pedestrians are dynamically assigned onto the road network via a traffic assignment model. Secondly, a nonlinear pedestrian road impedance function is introduced to address the congestion effects of massive crowds, and the pedestrian travel time changing rate is calculated for each link under various traffic volumes. It is proposed to sort the networks links according to the travel time changing rate. The rank is thus defined as a measurement of the structural importance of each link. Further, the structural importance is used to determine link robustness under different pedestrian traffic demand. Combing the result of structural importance and link robustness, bottleneck of the crowd circulating network can be identified. Finally, the Love Parade 2010 in Duisburg (an electronic music festival) is adopted as a case to illustrate the applicability of the proposed network bottleneck identification method. The threshold of pedestrian volume on the network and the effect of road control strategy are further investigated, the obtained basic data and theoretical results can benefit scientific planning and management of massive crowd road traffic.},
keyword={\textit{Keywords: }\textbf{Bottleneck identification;  Importance of network components;  Massive crowds;  Pedestrian road impedance function;  Transportation network}},
document_type={Article},
source={\textit{Source: }\textbf{Scopus}},
}

@CONFERENCE{Jian2015Evaluating,
timestamp={2017.05.29},
cat= {\textit{Category: }\textbf{PEDESTRIAN}},
author={Jian, M.a  and Chen, J.b  and Lo, S.b  and Xu, S.a  and Song, W.c },
title={Evaluating Bottleneck Magnitude of Massive Crowd Flow Networks},
journal={IEEE Conference on Intelligent Transportation Systems, Proceedings, ITSC},
year={2015},
volume={2015-October},
pages={1093-1097},
doi={10.1109/ITSC.2015.181},
art_number={7313273},
noteD={\textbf{Cited by 3(Scopus)/ 1(Google)}},
url2={http://ieeexplore.ieee.org/abstract/document/7313273/},
affiliation={National United Engineering Laboratory of Integrated and Intelligent Transportation, School of Transportation and Logistics, Southwest Jiaotong University, Chengdu, China; Department of Architecture and Civil Engineering, City University of Hong Kong, Hong Kong, Hong Kong; State Key Laboratory of Fire Science, University of Science and Technology of China, Hefei, China},
abstract={\textit{Abstract: }Under scenario of sports events and other kind of mass gathering, a large amount of people would travel along road networks, thus forming crowded pedestrians. In the crowds, the density would be so high that it might trigger mass panic and stampede, causing serious injuries and casualties. Therefore, it is necessary to understand pedestrian flow features on the corresponding network and then apply proper control method to organize and manage pedestrian flow. Firstly, considering general characteristics of travelers' route choice behavior, all these pedestrians are assigned onto the road network via a traffic assignment model. Secondly, a nonlinear pedestrian road impedance function is introduced to address the congestion effects of massive crowds, and the pedestrian travel time changing rate is calculated for each link under various traffic volumes. It is proposed to sort network links according to the travel time changing rate as an evaluation of the link bottleneck magnitude. Finally, the Love Parade 2010 in Duisburg (an electronic music festival) is adopted as a case study to illustrate the applicability of the proposed network bottleneck magnitude evaluating method.},
keyword={\textit{Keywords: }\textbf{}},
document_type={Conference Paper},
source={\textit{Source: }\textbf{Scopus}},
}

@CONFERENCE{Li2015continuum,
timestamp={2017.05.29},
author={Li, L.-Y.},
title={A continuum model of traffic flow on road networks},
journal={ICTIS 2015 - 3rd International Conference on Transportation Information and Safety, Proceedings},
year={2015},
pages={595-598},
doi={10.1109/ICTIS.2015.7232058},
art_number={7232058},
noteD={\textbf{Cited by 0}},
url2={http://ieeexplore.ieee.org/abstract/document/7232058/},
affiliation={School of Marine Science and Engineering, University of Plymouth, Plymouth, United Kingdom},
abstract={\textit{Abstract: }This paper presents a continuum model of traffic flow on a road network with taking into account the diffusion effect. The model is described by a nonlinear convection-dominant diffusion equation, which can be solved using numerical methods. The model is applied to analyzing the traffic flow along a unidirectional highway system with or without junctions. Three numerical examples are provided to illustrate the application of the present model.},
  keyword={\textit{Keywords: }\textbf{continuum model;  road network;  traffic}},
document_type={Conference Paper},
 source={\textit{Source: }\textbf{Scopus}},
}

@ARTICLE{Long2015intersection,
timestamp={2017.05.29},
author={Long, J.a  and Szeto, W.Y.b  and Huang, H.-J.c  and Gao, Z.d },
title={An intersection-movement-based stochastic dynamic user optimal route choice model for assessing network performance},
journal={Transportation Research Part B: Methodological},
year={2015},
volume={74},
pages={182-217},
doi={10.1016/j.trb.2014.12.008},
noteD={\textbf{Cited by 5(Scopus)/ 7(Google)}},
url2={http://www.sciencedirect.com/science/article/pii/S0191261514002252},
affiliation={School of Transportation Engineering, Hefei University of Technology, Hefei, China; Department of Civil Engineering, The University of Hong Kong, Pokfulam Road, Hong Kong; School of Economics and Management, Beihang University, Beijing, China; School of Traffic and Transportation, Beijing Jiaotong University, Beijing, China},
abstract={\textit{Abstract: }Different from traditional methods, this paper formulates the logit-based stochastic dynamic user optimal (SDUO) route choice problem as a fixed point (FP) problem in terms of intersection movement choice probabilities, which contain travelers' route information so that the realistic effects of physical queues can be captured in the formulation when a physical-queue traffic flow model is adopted, and that route enumeration and column generation heuristics can be avoided in the solution procedure when efficient path sets are used. The choice probability can be either destination specific or origin-destination specific, resulting into two formulations. To capture the effect of physical queues in these FP formulations, the link transmission model is modified for the network loading and travel time determination. The self-regulated averaging method (SRAM) was adopted to solve the FP formulations. Numerical examples were developed to illustrate the properties of the problem and the effectiveness of the solution method. The proposed models were further used to evaluate the effect of information quality and road network improvement on the network performance in terms of total system travel time (TSTT) and the cost of total vehicle emissions (CTVE). Numerical results show that providing better information quality, enhancing link outflow capacity, or constructing a new road can lead to poor network performance. © 2014 Elsevier Ltd.},
keyword={\textit{Keywords: }\textbf{Dynamic traffic assignment;  Fixed point problem;  Intersection movement;  Stochastic dynamic user optimal;  Vehicle emissions}},
document_type={Article},
 source={\textit{Source: }\textbf{Scopus}},
 }

@article{long2013intersection,
timestamp={2017.05.31},
  title={An intersection-movement-based dynamic user optimal route choice problem},
  author={Long, Jiancheng and Huang, Hai-Jun and Gao, Ziyou and Szeto, Wai Yuen},
  journal={Operations Research},
  volume={61},
  number={5},
  pages={1134--1147},
  year={2013},
  publisher={INFORMS},
  url2={http://pubsonline.informs.org/doi/abs/10.1287/opre.2013.1202},
  noteD={\textbf{Cited by 16(Google)}},
  abstract={\textit{Abstract: } In this paper a novel variational inequality (VI) formulation of the dynamic user optimal (DUO) route choice problem is proposed using the concept of approach proportion. An approach proportion represents the proportion of travelers that select a turning or through movement when leaving a node. Approach proportions contain travelers' route information so that the realistic effects of physical queues can be captured in a formulation when a physical-queue traffic flow model is adopted, and so that route enumeration and path-set generation can be avoided in the solution procedure. In addition, the simple structure of the approach proportion representation allows us to decompose the constraint set for solving large-scale DUO route choice problems. This paper also discusses the existence and uniqueness of the solutions to the VI problem and develops a solution algorithm based on the extragradient method to solve the proposed VI problem. This solution algorithm makes use of the decomposition property of the constraint set and is convergent if the travel time functions are pseudomonotone and Lipschitz continuous. It is not necessary to know the Lipschitz constant of the travel time functions in advance. Finally, numerical examples are given to demonstrate the properties of the proposed model and the performance of the solution algorithm.},
  keyword={\textit{Keywords: }\textbf{dynamic traffic assignment; dynamic user optimal; approach proportion; variational inequality; extragradient method}},
  source={\textit{Source: }\textbf{Google}}  
}


@ARTICLE{Chen2015model,
timestamp={2017.05.29},
cat= {\textit{Category: }\textbf{Parking}},
author={Chen, Q.a  and Wang, Y.b },
title={A model for dynamic parking choice of drivers},
journal={Promet - Traffic - Traffico},
year={2015},
volume={27},
number={5},
pages={365-377},
doi={10.7307/ptt.v27i5.1594},
noteD={\textbf{Cited by 1(Scopus)/ 2(Google)}},
url2={http://hrcak.srce.hr/file/220268},
affiliation={School of Traffic and Transportation Engineering, Central South University, Changsha, China; School of Public Administration, Central South University, Changsha, China},
abstract={\textit{Abstract: }Taking time-varying parking demands and supplies into account, this paper develops a dynamic parking choice model to simulate drivers’ searching for parking spaces between parking lots. In this study, each parking lot has one access passage and vehicles can move or wait for entering the park in the access passage. The flow propagation formula in the access passage of parking lots is established to obtain the number of vehicles entering the parking lot from the access passage within each time interval. This paper brings forward the instantaneous dynamic user-optimal condition of dynamic parking choice, constructs an equivalent variational inequality (VI) model and develops a diagonalization algorithm to solve the model. A numerical example demonstrates the rate of in-flow, the rate of out-flow, link flow, instantaneous travel time on each link or access passage of the parking lot, and the amount and routes of cruising traffic at each time point. © 2015, Faculty of Transport and Traffic Engineering.},
keyword={\textit{Keywords: }\textbf{Dynamic;  Parking;  User-optimal;  Variational inequality (VI)}},
document_type={Article},
source={\textit{Source: }\textbf{Scopus}}
}


@ARTICLE{Jiang2014Macroscopic,
timestamp={2017.05.29},
author={Jiang, Y.Q.a  and Zhou, S.G.b },
title={Macroscopic simulation of traffic flow on continuum urban networks},
journal={Applied Mechanics and Materials},
year={2014},
volume={641-642},
pages={887-891},
doi={10.4028/www.scientific.net/AMM.641-642.887},
noteD={\textbf{Cited by 0}},
url2={http://www.scientific.net/AMM.641-642.887},
affiliation={Department of Mathematics, Southwest University of Science and Technology, Mianyang, China; China Aerodynamics Research and Development Center, Mianyang, China},
abstract={\textit{Abstract: }In this paper, a macroscopic model is applied to simulate dynamical features of traffic flow on a continuum urban network. This model is described as the two-dimensional Lighthill-Whitham-Richards model coupled with a reactive dynamic user-optimal route choice model. Numerical results visualize the ability of the model to predict some macroscopic characteristics of traffic flow on networks, i.e. the spatial distribution of flow density and travel cost of users, as well as to capture traffic congestion build-up and dissipation.},
keyword={\textit{Keywords: }\textbf{Finite volume method;  Macroscopic model;  Traffic congestion;  Traffic flow;  Urban network}},
document_type={Conference Paper},
source={\textit{Source: }\textbf{Scopus}},
}

@ARTICLE{Duan2014Real,
timestamp={2017.05.29},
author={Duan, Z.-T.a  b  and Li, Y.a  and Zheng, X.-B.a  and Kang, J.a  b  and Cheng, H.a },
title={Real-time multi-path traffic flow assignment algorithm based on Hadoop platform},
journal={Zhongguo Gonglu Xuebao/China Journal of Highway and Transport},
year={2014},
volume={27},
number={9},
pages={98-104},
noteD={\textbf{Cited by 1, No PDF Available}},
url2={https://goo.gl/ocuv3C},
affiliation={School of Information Engineering, Chang'an University, Xi'an, Shaanxi, China; Shaanxi Road Traffic Intelligent Detection and Equipment Engineering Technology Research Center, Chang'an University, Xi'an, Shaanxi, China},
abstract={\textit{Abstract: }The equilibrium of traffic flow based on the traditional traffic flow assignment algorithms is hard to guarantee. To solve this problem, Hadoop big data computing platform was adopted for designing and implementing a real-time multi-path traffic flow assignment algorithm. If there were more than one paths with the minimum impedance between the purposed OD pairs, a set of all minimum impedance paths between the OD pairs would be found out firstly. Then, the traffic flow on the OD pairs would be uniformly assigned to the set of paths so as to avoid exceeding of actual traffic flow in each section beyond its capacity threshold, and prevent the delayed congestion. At last, a simulation of the real-time multi-path traffic flow assignment algorithm based on Hadoop big data computing platform was made. The results show that compared with traditional methods, the traffic flow of each section at each moment in the simulated road network decreases by 42.3\% averagely, the mean square deviation decreases by 35.8\% averagely, and the maximum traffic flow decreases by 19.4\% averagely.},
keyword={\textit{Keywords: }\textbf{Equilibrium of traffic flow;  Hadoop platform;  Model simulation;  OD pair;  Traffic engineering;  Traffic flow assignment;  Traffic guidance}},
document_type={Article},
source={\textit{Source: }\textbf{Scopus}},
}

@ARTICLE{Tao2014Dynamic,
timestamp={2017.05.29},
author={Tao, Y.Z.a  and Jiang, Y.Q.b  and Du, J.c  and Wong, S.C.d  and Zhang, P.a  and Xia, Y.H.c  and Choi, K.e },
title={Dynamic system-optimal traffic assignment for a city using the continuum modeling approach},
journal={Journal of Advanced Transportation},
year={2014},
volume={48},
number={7},
pages={782-797},
doi={10.1002/atr.1227},
noteD={\textbf{Cited by 1(Scopus)/ 4(Google)}},
url2={http://onlinelibrary.wiley.com/doi/10.1002/atr.1227/full},
affiliation={Shanghai Institute of Applied Mathematics and Mechanics, Shanghai University, Shanghai, China; Department of Mathematics, Southwest University of Science and Technology, Mianyang, Sichuan, China; Department of Mathematics, University of Science and Technology of China, Hefei, Anhui, China; Department of Civil Engineering, University of Hong Kong, Pokfulam Road, Hong Kong, Hong Kong; Department of Transportation Engineering, TOD-based Sustainable Urban Transportation Center, Ajou University, South Korea},
abstract={\textit{Abstract: }This paper presents a continuum dynamic traffic assignment model for a city in which the total cost of the traffic system is minimized: the travelers in the system are organized to choose the route to their destinations that minimizes the total cost of the system. Combined with the objective function, which defines the total cost and constraints such as certain physical and boundary conditions, a continuum model can be formulated as an optimization scheme with a feasible region in the function space. To obtain an admissible locally optimal solution to this problem, we first reformulate the optimization in discrete form and then introduce a heuristic method to solve it. This method converges rapidly with attractive computational cost. Numerical examples are used to demonstrate the effectiveness of the method.},
keyword={\textit{Keywords: }\textbf{continuum model;  dynamic system optimal;  heuristic method}},
document_type={Article},
source={\textit{Source: }\textbf{Scopus}},
}

@ARTICLE{Du2013Revisiting,
timestamp={2017.05.29},
author={Du, J.a  and Wong, S.C.b  and Shu, C.-W.c  and Xiong, T.d  and Zhang, M.a  and Choi, K.e },
title={Revisiting Jiang's dynamic continuum model for urban cities},
journal={Transportation Research Part B: Methodological},
year={2013},
volume={56},
pages={96-119},
doi={10.1016/j.trb.2013.07.001},
noteD={\textbf{Cited By 7(Scopus)/ 10(Google)}},
url2={http://www.sciencedirect.com/science/article/pii/S0191261513001161},
affiliation={Department of Mathematics, University of Science and Technology of China, Hefei, Anhui, China; Department of Civil Engineering, The University of Hong Kong, Pokfulam Road, Hong Kong, China; Division of Applied Mathematics, Brown University, Providence, RI, United States; Department of Mathematics, University of Houston, Houston, TX, United States; Department of Transportation Engineering, TOD-based Sustainable Urban Transportation Center, Ajou University, South Korea},
abstract={\textit{Abstract: }Jiang et al. (Jiang, Y.Q., Wong, S.C., Ho, H.W., Zhang, P., Liu, R.X., Sumalee, A., 2011. A dynamic traffic assignment model for a continuum transportation system. Transportation Research Part B 45 (2), 343-363) proposed a predictive continuum dynamic user-optimaDUO-l to investigate the dynamic characteristics of traffic flow and the corresponding route-choice behavior of travelers. Their modeled region is a dense urban city that is arbitrary in shape and has a single central business district (CBD). However, we argue that the model is not well posed due to an inconsistency in the route-choice strategy under certain conditions. To overcome this inconsistency, we revisit the PDUO-C problem, and construct an improved path-choice strategy. The improved model consists of a conservation law to govern the density, in which the flow direction is determined by the improved path-choice strategy, and a Hamilton-Jacobi equation to compute the total travel cost. The simultaneous satisfaction of both equations can be treated as a fixed-point problem. A self-adaptive method of successive averages (MSA) is proposed to solve this fixed-point problem. This method can automatically determine the optimal MSA step size using the least squares approach. Numerical examples are used to demonstrate the effectiveness of the model and the solution algorithm. © 2013 Elsevier Ltd.},
keyword={\textit{Keywords: }\textbf{Conservation law;  Continuum model;  Dynamic traffic assignment;  Hamilton-Jacobi equation;  Path-choice strategy;  Predictive user equilibrium}},
document_type={Article},
source={\textit{Source: }\textbf{Scopus}},
}

@ARTICLE{Zheng2013distribution,
timestamp={2017.05.29},
author={Zheng, N. and Geroliminis, N.},
title={On the distribution of urban road space for multimodal congested networks},
journal={Transportation Research Part B: Methodological},
year={2013},
volume={57},
pages={326-341},
doi={10.1016/j.trb.2013.06.003},
noteD={\textbf{Cited By 18(Scopus)/ 38(Google)}},
url2={http://www.sciencedirect.com/science/article/pii/S1877042813009786},
affiliation={School of Architecture, Civil and Environmental Engineering, Laboratory of Urban Transport Systems, École Polytechnique Fédérale de Lausanne (EPFL), Switzerland},
abstract={\textit{Abstract: }Transport systems in real cities are complex with many modes of transport sharing and competing for limited road space. This work intends to understand how space distributions for modes and interactions among modes affect network traffic performance. While the connection between performance of transport systems and general land allocation is the subject of extensive research, space allocation for interacting modes of transport is an open research question. Quantifying the impact of road space distribution on the performance of a congested multimodal transport system with a dynamic aggregated model remains a challenge. In this paper, a multimodal macroscopic fundamental diagram (MFD) is developed to represent the traffic dynamics of a multimodal transport system. Optimization is performed with the objective of minimizing the total passenger hours traveled (PHT) to serve the total demand by redistributing road space among modes. Pricing strategies are also investigated to provide a higher demand shift to more efficient modes. We find by an application to a bi-modal two-region city that (i) the proposed model captures the operational characteristics of each mode, and (ii) optimal dynamic space distribution strategies can be developed. In practice, the approach can serve as a physical dynamic model to inform space distribution strategies for policy makers with different goals of mobility. © 2013 Elsevier Ltd.},
keyword={\textit{Keywords: }\textbf{Macroscopic fundamental diagram;  Multi-modal;  Optimization;  Public transport;  Space allocation;  Traffic flow}},
document_type={Article},
source={\textit{Source: }\textbf{Scopus}},
}

@CONFERENCE{Peng2012Macroscopic,
timestamp={2017.05.29},
author={Peng, J. and Wong, S.C.},
title={Macroscopic properties of dense road networks},
journal={Proceedings of the 17th International Conference of Hong Kong Society for Transportation Studies, HKSTS 2012: Transportation and Logistics Management},
year={2012},
pages={99-106},
noteD={\textbf{Cited by 0, No PDF Available}},
url2={http://hub.hku.hk/handle/10722/180305},
affiliation={Department of Civil Engineering, University of Hong Kong, China},
abstract={\textit{Abstract: }Recent empirical evidence has shown that the relationships between speed, flow and density on highway sections are also observable on general networks. In this study, we extend the Bureau of Public Roads Function (BPRF) and the Fundamental Diagram of Road Traffic (FDRT) relationships to represent the macroscopic properties of dense road networks. Road networks with an area of 1 km by 1 km are cordoned from the Hong Kong road system. The origin-destination (OD) matrices are multiplied by scaling factors to generate different traffic conditions. These scenarios are simulated using the microscopic simulation package (VISSIM) based on dynamic traffic assignment. The simulation results are then collected to construct a Macroscopic Bureau of Public Roads Function (MBPRF) and Macroscopic Fundamental Diagrams of Road Traffic (MFDRT). The relationships between the macroscopic parameters and network attributes such as road density and the number of junctions are presented to illustrate the macroscopic properties of dense road networks.},
keyword={\textit{Keywords: }\textbf{Bureau of Public Roads Function;  Macroscopic fundamental diagram;  Micro-simulation}},
document_type={Conference Paper},
source={\textit{Source: }\textbf{Scopus}},
}

@ARTICLE{Szeto2012Road,
timestamp={2017.05.29},
cat= {\textit{Category: }\textbf{ENVIRONMENT}},
author={Szeto, W.Y. and Jaber, X. and Wong, S.C.},
title={Road Network Equilibrium Approaches to Environmental Sustainability},
journal={Transport Reviews},
year={2012},
volume={32},
number={4},
pages={491-518},
doi={10.1080/01441647.2012.690000},
noteD={\textbf{Cited By 34(Scopus)/ 50(Google)}},
url2={http://www.tandfonline.com/doi/abs/10.1080/01441647.2012.690000},
affiliation={Department of Civil Engineering, The University of Hong Kong, Hong Kong, China},
abstract={\textit{Abstract: }Environmental sustainability is closely related to transportation, especially to the road network, because vehicle emissions and noise damage the environment and have adverse effects on human health. It is, therefore, important to take their effect into account when designing and managing road networks. Road network equilibrium approaches have been used to estimate this impact and to design and manage road networks accordingly. However, no comprehensive review has summarized the applications of these approaches to the design and management of road networks that explicitly address environmental concerns. More importantly, it is necessary to identify this gap in the literature so that future research can improve the existing methodologies. Hence, this paper summarizes these applications and identifies potential future research directions in terms of theories, modelling approaches, algorithms, analyses, and applications.},
keyword={\textit{Keywords: }\textbf{No keywords}},

document_type={Article},
source={\textit{Source: }\textbf{Scopus}},

}

@ARTICLE{Szeto2012Dynamic,
timestamp={2017.05.29},
author={Szeto, W.Y. and Wong, S.C.},
title={Dynamic traffic assignment: Model classifications and recent advances in travel choice principles},
journal={Central European Journal of Engineering},
year={2012},
volume={2},
number={1},
pages={1-18},
doi={10.2478/s13531-011-0057-y},
noteD={\textbf{Cited By 18(Scopus)/ 29(Google)}},
url2={http://link.springer.com/article/10.2478/s13531-011-0057-y},
affiliation={Department of Civil Engineering, University of Hong Kong, Hong Kong, Hong Kong},
abstract={\textit{Abstract: }Dynamic Traffic Assignment (DTA) has been studied for more than four decades and numerous reviews of this research area have been conducted. This review focuses on the travel choice principle and the classification of DTA models, and is supplementary to the existing reviews. The implications of the travel choice principle for the existence and uniqueness of DTA solutions are discussed, and the interrelation between the travel choice principle and the traffic flow component is explained using the nonlinear complementarity problem, the variational inequality problem, the mathematical programming problem, and the fixed point problem formulations. This paper also points out that all of the reviewed travel choice principles are extended from those used in static traffic assignment. There are also many classifications of DTA models, in which each classification addresses one aspect of DTA modeling. Finally, some future research directions are identified. © Versita sp. z o.o.},
keyword={\textit{Keywords: }\textbf{Departure time choice;  Dynamic traffic assignment;  Route choice;  User equilibrium}},
document_type={Article},
source={\textit{Source: }\textbf{Scopus}},
}

@ARTICLE{Jiang2011Macroscopic,
timestamp={2017.05.29},
key={PEDESTRIAN},
author={Jiang, Y.a  and Zhang, P.b },
title={Macroscopic simulation of pedestrian flow through a bottleneck},
journal={Applied Mechanics and Materials},
year={2011},
volume={97-98},
pages={1168-1175},
doi={10.4028/www.scientific.net/AMM.97-98.1168},
noteD={\textbf{Cited By 1(Scopus)/ 0(Google)}},
url2={http://www.scientific.net/AMM.97-98.1168},
affiliation={Department of Mathematics, Southwest University of Science and Technology, Mianyang 621010, Sichuan, China; Shanghai Institute of Applied Mathematics and Mechanics, Shanghai University, Shanghai 200072, China},
abstract={\textit{Abstract: }The paper deals with the macroscopic type modelling of the unidirectional pedestrian flow moving through a corridor with a bottleneck. The macroscopic model of pedestrian flow is the two-dimensional Lighthill-Whitham-Richards model described as a mass conservation equation. The characteristic feature of pedestrian route choice is that pedestrians in the corridor try to minimize the instantaneous travel time and improve the comfort level. The model equation is solved numerically by the discontinuous Galerkin method. Numerical results visualize the ability of the model to predict macroscopic characteristics of pedestrian flow through bottlenecks, i.e. the spatial distribution of the flow speed and density, as well as the formation and dissipation of traffic congestion in the corridor. They also validate that congestion is caused by the limited capacity of the bottleneck. © (2011) Trans Tech Publications.},
keyword={\textit{Keywords: }\textbf{Bottleneck;  Discontinuous Galerkin method;  Macroscopic pedestrian flow;  Route choice;  Traffic congestion}},
document_type={Conference Paper},
source={\textit{Source: }\textbf{Scopus}},
}

@ARTICLE{Long2017dynamic,
timestamp={2017.05.29},
key={TAXI},
author={Long, J.a  and Szeto, W.Y.b  and Du, J.c  and Wong, R.C.P.b },
title={A dynamic taxi traffic assignment model: A two-level continuum transportation system approach},
journal={Transportation Research Part B: Methodological},
year={2017},
volume={100},
pages={222-254},
doi={10.1016/j.trb.2017.02.005},
noteD={\textbf{Cited By 0(Scopus)/ 0(Google)}},
url2={http://www.sciencedirect.com/science/article/pii/S0191261516304672},
affiliation={School of Automotive and Transportation Engineering, Hefei University of Technology, Hefei, China; Department of Civil Engineering, The University of Hong Kong, Pokfulam Road, Hong Kong; Department of Mathematics, The Chinese University of Hong Kong, Shatin, NT, Hong Kong},
abstract={\textit{Abstract: }This paper proposes a two-level continuum transportation system approach to modeling a dynamic taxi traffic assignment (DTTA) problem in a dense network with real-time traffic information provision and three types of vehicles, including private cars, occupied taxis, and vacant taxis. The proposed approach treats the dense network as a continuum in the first level, in which private car and occupied taxi drivers are free to choose their paths in a two-dimensional continuous space. The proposed approach also divides the modeling region into many identical squares to form a cell-based network in the second level, in which the cells are classified into two categories: target cell with an acceptable expected rate of return (EROR) to vacant taxi drivers and non-target cell with an unacceptable EROR. The EROR associated with a cell is the ratio of the cumulative expected profit of a taxi driver who successfully picks up a customer during the customer search that starts from that cell to the sum of expected search time for this customer and expected occupied travel time to serve this customer. Based on the cell-based network, we develop a cell-based intervening opportunity model to capture the fact that vacant taxi drivers can meet a customer on the way to their destination zones and estimate the EROR. Each vacant taxi driver has a mixed strategy to determine his/her customer-search direction according to the EROR: Each vacant taxi driver in a target cell selects its neighbor cells with maximum EROR, and each vacant taxi driver in a non-target cell selects the travel time-based shortest path to his/her target cell. Meanwhile, each private car driver chooses the path that minimizes his/her own generalized travel cost, and each occupied taxi driver chooses the path that minimizes his/her customer's generalized in-vehicle travel cost. In our model, traffic density in the system is governed by the conservation law (CL), and the flow directions of different vehicles are determined by the path-choice strategies of their drivers, which are captured by Hamilton–Jacobi (HJ) equations. Both the proposed CL and HJ equations can be solved by the Lax–Friedrichs scheme, which forms the backbone of the developed solution algorithm. Finally, numerical examples and a case study are used to demonstrate the properties of the model, the performance of the solution algorithm, and the value of using our methodology for estimating network performance. © 2017 Elsevier Ltd},
keyword={\textit{Keywords: }\textbf{Conservation law;  Continuum model;  Hamilton–Jacobi equation;  Intervening opportunity model;  Reactive dynamic user optimal;  Taxi customer-search}},
document_type={Article},
source={\textit{Source: }\textbf{Scopus}},
}



@ARTICLE{Du2016multi,
timestamp={2017.05.29},
author={Du, Y.C.a  and Wong, S.C.b  and Sun, L.J.a },
title={A multi-commodity discrete/continuum model for a traffic equilibrium system},
journal={Transportmetrica A: Transport Science},
year={2016},
volume={12},
number={3},
pages={249-271},
doi={10.1080/23249935.2015.1128011},
noteD={\textbf{Cited By 1(Scopus)/ 2(Google)}},
url2={http://www.tandfonline.com/doi/abs/10.1080/23249935.2015.1128011},
affiliation={Key Laboratory of Road and Traffic Engineering of the Ministry of Education, Tongji University, Shanghai, China; Department of Civil Engineering, The University of Hong Kong, Hong Kong},
abstract={\textit{Abstract: }We consider a city with several highly compact central business districts (CBDs). The commuters’ origins are continuously dispersed. The travel demand to each CBD, which is considered to be a distinct commodity of traffic movements, is dependent on the total travel cost to that CBD. The transportation system is divided into two layers: major freeways and a dense network of surface streets. Whereas the major freeway network is modelled according to the conventional discrete-network approach, the dense surface streets are approximated as a continuum. Travellers to each CBD can either travel within the continuum (surface streets) and then transfer to the discrete network (freeways) at an interchange (ramp) before moving to the CBD on the discrete network, or they can travel directly to the CBD within the continuum. Specific travel cost-flow relationships for the two layers of transportation facilities are considered. We develop a traffic equilibrium model for this discrete/continuum transportation system in which, for each origin–destination pair, no traveller can reduce his or her individual travel cost by unilaterally changing routes. The problem is formulated as a simultaneous optimisation programme with two sub-problems. One sub-problem is a traffic assignment problem from the interchanges to the CBD in the discrete network, and the other is a traffic assignment problem within a continuum system with multiple centres (i.e. the interchange points and the CBDs). A Newtonian algorithm based on sensitivity analyses of the two sub-problems is proposed to solve the resultant simultaneous optimisation programme. A numerical example is given to demonstrate the effectiveness of the proposed method. © 2016 Hong Kong Society for Transportation Studies Limited.},
keyword={\textit{Keywords: }\textbf{continuum system;  Discrete system;  elastic demand;  multi-commodity;  traffic equilibrium}},
document_type={Article},
source={\textit{Source: }\textbf{Scopus}},
}

@ARTICLE{Jiang2016Comparison,
timestamp={2017.05.29},
key={PEDESTRIAN},
author={Jiang, Y.-Q.a  and Zhang, W.b  and Zhou, S.-G.c },
title={Comparison study of the reactive and predictive dynamic models for pedestrian flow},
journal={Physica A: Statistical Mechanics and its Applications},
year={2016},
volume={441},
pages={51-61},
doi={10.1016/j.physa.2015.08.047},
art_number={16364},
noteD={\textbf{Cited By 1(Scopus)/ 2(Google)}},
url2={http://www.sciencedirect.com/science/article/pii/S0378437115007128},
affiliation={Department of Mathematics, Southwest University of Science and Technology, Mianyang, Sichuan, China; School of Civil Engineering and Architecture, Southwest University of Science and Technology, Mianyang, Sichuan, China; China Aerodynamics Research and Development Center, Mianyang, Sichuan, China},
abstract={\textit{Abstract: }This paper formulates the reactive and predictive dynamic models for pedestrian flow and presents a comparison of the two models. The path-choice behavior of pedestrians in the reactive dynamic model is described that pedestrians tend to walk along a path with the lowest instantaneous cost. The desired walking direction of pedestrians in the predictive dynamic model is chosen to minimize the actual cost based on predictive traffic conditions. An algorithm used to solve the two models encompasses a cell-centered finite volume method for a hyperbolic system of conservation laws and a time-dependent Hamilton-Jacobi equation, a fast sweeping method for an Eikonal-type equation, and a self-adaptive method of successive averages for an arisen discrete fixed point problem. The two models and their algorithm are applied to investigate the spatio-temporal patterns of flux or density and path-choice behaviors of pedestrian flow marching in a facility scattered with an obstacle. Numerical results show that the two models are able to capture macroscopic features of pedestrian flow, traffic instability and other complex nonlinear phenomena in pedestrian traffic, such as the formation of stop-and-go waves and clogging at bottlenecks. Different path-choice strategies of pedestrians cause different spatial distributions of pedestrian density specially in the high-density regions (near the obstacle and exits). © 2015 Elsevier B.V.},
keyword={\textit{Keywords: }\textbf{Pedestrian flow;  Predictive dynamic user-equilibrium;  Reactive dynamic user-equilibrium;  Stop-and-go waves;  Traffic instability}},
document_type={Article},
source={\textit{Source: }\textbf{Scopus}},
}

@ARTICLE{Du2015Reformulating,
timestamp={2017.05.29},
author={Du, J.a  and Wong, S.C.b  and Shu, C.-W.c  and Zhang, M.a },
title={Reformulating the Hoogendoorn-Bovy predictive dynamic user-optimal model in continuum space with anisotropic condition},
journal={Transportation Research Part B: Methodological},
year={2015},
volume={79},
pages={189-217},
doi={10.1016/j.trb.2015.06.005},
noteD={\textbf{Cited By 2(Scopus)/ 3(Google)}},
url2={http://www.sciencedirect.com/science/article/pii/S0191261515001289},
affiliation={School of Mathematical Sciences, University of Science and Technology of China, Hefei, Anhui, China; Department of Civil Engineering, The University of Hong Kong, Pokfulam Road, Hong Kong, China; Division of Applied Mathematics, Brown University, Providence, RI, United States},
abstract={\textit{Abstract: }Hoogendoorn and Bovy (2004) developed an approach for a pedestrian user-optimal dynamic assignment in continuous time and space. Although their model was proposed for pedestrian traffic, it can also be applied to urban cities. The model is very general, and consists of a conservation law (CL) and a Hamilton-Jacobi-Bellman (HJB) equation that contains a minimum value problem. However, only an isotropic application example was given in their paper. We claim that the HJB equation is difficult to compute numerically in an anisotropic case. To overcome this, we reformulate their model for a dense urban city that is arbitrary in shape and has multiple central business districts (CBDs). In our model, the minimum value problem is only used in the CL portion, and the HJB equation reduces to a Hamilton-Jacobi (HJ) equation for easier computation. The dynamic path equilibrium of our model is proven in a different way from theirs, and a numerical algorithm is also provided to solve the model. Finally, we show two numerical examples under the anisotropic case and compare the results with those of the isotropic case. © 2015 Elsevier Ltd.},
keyword={\textit{Keywords: }\textbf{Anisotropic;  Conservation law;  Continuum model;  Dynamic traffic assignment;  Hamilton-Jacobi equation;  Predictive user equilibrium}},
document_type={Article},
source={\textit{Source: }\textbf{Scopus}},
}

@ARTICLE{Mounce2015convergence,
timestamp={2017.05.29},
author={Mounce, R.a  and Carey, M.b  c },
title={On the convergence of the method of successive averages for calculating equilibrium in traffic networks},
journal={Transportation Science},
year={2015},
volume={49},
number={3},
pages={535-542},
doi={10.1287/trsc.2014.0517},
noteD={\textbf{Cited By 4(Scopus)/ 4(Google)}},
url2={http://pubsonline.informs.org/doi/abs/10.1287/trsc.2014.0517},
affiliation={Centre for Transport Research, University of Aberdeen, Aberdeen, United Kingdom; Institute for Transport Studies, University of Leeds, Leeds, United Kingdom; Ulster Business School, University of Ulster, Belfast, United Kingdom},
abstract={\textit{Abstract: }The traffic assignment problem aims to calculate an equilibrium route flow vector, generally by seeking a zero of an appropriate objective function. If a continuous dynamical system follows a descent direction for this objective function at each nonequilibrium route flow vector, the system converges to equilibrium. It is shown that when this dynamical system is discretized with a fixed step length, the system eventually approaches close to equilibrium provided that the objective function is continuously differentiable and that the rate of descent is bounded below. The method of successive averages is widely used in traffic assignment; it has a decreasing step size at each iteration. With the same conditions as above, it is shown that the resulting dynamical system converges to equilibrium. In the steady-state model, the necessary conditions are shown to be satisfied, provided that the route cost vector is a continuously differentiable monotone function of the route flow vector. However, continuous differentiability of the cost function is shown not to hold in the dynamic queueing model. © 2015 INFORMS.},
keyword={\textit{Keywords: }\textbf{Equilibrium;  Method of successive averages;  Step length;  Traffic assignment}},
document_type={Article},
source={\textit{Source: }\textbf{Scopus}},
}

@ARTICLE{Yildirimoglu2014Approximating,
timestamp={2017.05.29},
author={Yildirimoglu, M. and Geroliminis, N.},
title={Approximating dynamic equilibrium conditions with macroscopic fundamental diagrams},
journal={Transportation Research Part B: Methodological},
year={2014},
volume={70},
pages={186-200},
doi={10.1016/j.trb.2014.09.002},
noteD={\textbf{Cited By 18(Scopus)/ 27(Google)}},
url2={http://www.sciencedirect.com/science/article/pii/S0191261514001568},
affiliation={School of Architecture, Civil and Environmental Engineering, Urban Transport Systems Laboratory, Ecole Polytechnique Fédérale de Lausanne (EPFL), GC C2 406, Station 18, Lausanne, Switzerland},
abstract={\textit{Abstract: }Real-time coordinated traffic management strategies that benefit from parsimonious models with aggregated network dynamics, provide a new generation of smart hierarchical strategies to improve network capacity and performance. However, this raises the question of route choice behavior in case of heterogeneous urban networks, where different parts of the city are subject to different types of control. Traffic equilibrium phenomena have not been thoroughly investigated in these models. Approximate traffic equilibrium conditions can be integrated within the parsimonious traffic models to develop regional routing strategies, while detailed route choice strategies can be incorporated at a later stage in a hierarchical framework. In this study, we develop an aggregated and approximate dynamic traffic assignment (DTA) procedure to be incorporated in the macroscopic fundamental diagram (MFD) dynamics, and establish dynamic stochastic user equilibrium (DSUE) conditions. The methodology consists of two main components; stochastic network loading and a fixed-point solution method. Loading procedure is designed to handle stochastic components in the model such as trip length uncertainty, variation of speeds across the links, perception error of travelers. The results taken from this procedure are averaged through the well-known method of successive averages (MSA) to reach fixed-point solution for the system. Real-time route guidance strategies can be revisited towards a "system of systems" approach.},
keyword={\textit{Keywords: }\textbf{Dynamic stochastic user equilibrium;  Dynamic traffic assignment;  Macroscopic fundamental diagram}},
source={\textit{Source: }\textbf{Scopus}},
}

@article{HUANG2009Revisiting,
timestamp={2017.06.02},
cat= {\textit{Category: }\textbf{PEDESTRIAN}},
title = {Revisiting Hughes’ dynamic continuum model for pedestrian flow and the development of an efficient solution algorithm},
author = {Ling Huang and S.C. Wong and Mengping Zhang and Chi-Wang Shu and William H.K. Lam},
journal = {Transportation Research Part B: Methodological},
volume = {43},
number = {1},
pages = {127 - 141},
year = {2009},
noteD={\textbf{Cited by 162(Google)}},
issn = {0191-2615},
doi = {http://dx.doi.org/10.1016/j.trb.2008.06.003},
url2 = {http://www.sciencedirect.com/science/article/pii/S0191261508000751},
abstract={\textit{Abstract: }In this paper, we revisit Hughes’ dynamic continuum model for pedestrian flow in a two-dimensional walking facility that is represented as a continuum within which pedestrians can freely move in any direction [Hughes, R.L., 2002. A continuum theory for the flow of pedestrians. Transportation Research Part B, 36 (6), 507–535]. We first reformulate Hughes’ model, and then show that the pedestrian route choice strategy in Hughes’ model satisfies the reactive dynamic user equilibrium principle in which a pedestrian chooses a route to minimize the instantaneous travel cost to the destination. In this model, the pedestrian demand is time varying. The pedestrian density, flux, and walking speed are governed by the conservation equation. A generalized cost function is considered. The reformulated problem is solved by the efficient weighted essentially non-oscillatory scheme for the conservation equation and the fast sweeping method for the Eikonal equation. A numerical example is used to demonstrate the effectiveness of the proposed solution procedure.},
keyword={\textit{Keywords: }\textbf{Pedestrian flow, Continuum modeling, Reactive dynamic user equilibrium, WENO scheme, Eikonal equation}},
source={\textit{Source: }\textbf{Dr. Laval}}
}

@article{JIANG2011Dynamic,
timestamp= {2017.06.02},
cat= {\textit {Category: }\textbf{ }},
title = {A dynamic traffic assignment model for a continuum transportation system},
author = {Yanqun Jiang and S.C. Wong and H.W. Ho and Peng Zhang and Ruxun Liu and Agachai Sumalee},
journal = {Transportation Research Part B: Methodological},
volume = {45},
number = {2},
pages = {343 - 363},
year = {2011},
noteD= {\textbf {Cited by 29(Google)}},
issn = {0191-2615},
doi = {http://dx.doi.org/10.1016/j.trb.2010.07.003},
url2 = {http://www.sciencedirect.com/science/article/pii/S0191261510000986},
abstract={\textit{Abstract: }A predictive continuum dynamic user-optimal (PDUO-C) model is formulated in this study to investigate the dynamic characteristics of traffic flow and the corresponding route-choice behavior of travelers within a region with a dense urban road network. The modeled region is arbitrary in shape with a single central business district (CBD) and travelers continuously distributed over the region. Within this region, the road network is represented as a continuum and travelers patronize a two-dimensional continuum transportation system to travel to the CBD. The PDUO-C model is solved by a promising solution algorithm that includes elements of the finite volume method (FVM), the finite element method (FEM), and the explicit total variation diminishing Runge–Kutta (TVD-RK) time-stepping method. A numerical example is given to demonstrate the utility of the proposed model and the effectiveness of the solution algorithm in solving this PDUO-C problem.},
keyword={\textit{Keywords: }\textbf{Continuum model, Dynamic traffic assignment, Predictive user-equilibrium, Path-choice strategy, Hamilton–Jacobi equation, Finite element method}},
source= {\textit {Source: }\textbf{Dr. Laval}}
}

@article{Hoogendoorn2004Dynamic,
timestamp={2017.06.02},
cat= {\textit{Category: }\textbf{PEDESTRIAN}},
title = {Dynamic user-optimal assignment in continuous time and space },
author = {Serge P. Hoogendoorn and Piet H.L. Bovy},
journal = {Transportation Research Part B: Methodological },
volume = {38},
number = {7},
pages = {571 - 592},
year = {2004},
noteD={\textbf{Cited by 82(Google)}},
issn = {0191-2615},
doi = {https://doi.org/10.1016/j.trb.2002.12.001},
url2 = {http://www.sciencedirect.com/science/article/pii/S0191261503000626},
abstract={\textit{Abstract: }To support planning, design, and management of pedestrian infrastructure, dynamic assignment models are useful tools. However, current models are network-based and presume that travelers can choose between a finite number of discrete route alternatives. For walking facilities, where pedestrians can choose their paths freely in two-dimensional space, applicability of these traditional network models is limited. This article puts forward an approach for user-optimal dynamic assignment in continuous time and space. Contrary to network-based approaches, the theory allows the traffic units to choose from an infinite non-countable set of paths through the considered space. The approach consists of three interrelated steps, that is: determining the continuous paths using a path choice model, assigning the origin–destination flows, and calculating the resulting traffic conditions. The approach to determine a user-optimal assignment is heuristic and consists of a sequence of all-or-nothing assignments in continuous time-space. The article presents the mathematical problem formulation, solution approaches, and application examples.},
keyword={\textit{Keywords: }\textbf{Dynamic assignment, Path-choice models, Pedestrian traffic, Continuous space models}},
source={\textit{Source: }\textbf{Dr. Laval}}
}

@Inbook{Sossoe2017Reactive,
timestamp={2017.06.06},
author={Sossoe, Kwami Seyram
and Lebacque, Jean Patrick},
editor={{\'{S}}wi{\k{a}}tek, Jerzy
and Tomczak, Jakub M.},
title={Reactive Dynamic Assignment for a Bi-dimensional Traffic Flow Model},
bookTitle={Advances in Systems Science: Proceedings of the International Conference on Systems Science 2016 (ICSS 2016)},
year={2017},
publisher={Springer International Publishing},
address={Cham},
pages={179--188},
isbn={978-3-319-48944-5},
keyword={\textit{Keywords: }\textbf{Reactive assignment; Cross-entropy algorithm; Traffic control; Continuum anisotropic network; Zone-based model of flow}},
cat= {\textit{Category: }\textbf{}},
noteD={\textbf{Cited by 0}},
source={\textit{Source: }\textbf{Dr. Laval}},
abstract={\textit{Abstract: }This paper develops a graph-theoretic framework for large scale bi-dimensional transport networks and provides new insight into the dynamic traffic assignment. Reactive dynamic assignment are deployed to handle the traffic contingencies, traffic uncertainties and traffic congestion. New shortest paths problem in large networks is defined and routes cost calculation is provided. Since mathematical modelling of traffic flow is a keystone in the theory of traffic flow management, and then in the traffic assignment, it is convenient to elaborate a good model of assignment for large scale networks relying on an appropriate model of flow related to very large networks. That is the zone-based optimization of traffic flow model on networks developed by [8], completed and improved by [9].},

}

@article{Hughes2002Continuum,
timestamp={2017.06.07},
cat= {\textit{Category: }\textbf{Pedestrian}},
noteD={\textbf{Cited by 709}},
source={\textit{Source: }\textbf{Dr. Laval}},
title = {A continuum theory for the flow of pedestrians},
journal = {Transportation Research Part B: Methodological},
volume = {36},
number = {6},
pages = {507 - 535},
year = {2002},
noteD = {},
issn = {0191-2615},
doi = {http://dx.doi.org/10.1016/S0191-2615(01)00015-7},
url2 = {http://www.sciencedirect.com/science/article/pii/S0191261501000157},
author = {Roger L. Hughes},
abstract={\textit{Abstract: }The equations of motion governing the two-dimensional flow of pedestrians are derived for flows of both single and multiple pedestrian types. Two regimes of flow, a high-density (subcritical) and a low-density (supercritical) flow regimes, are possible, rather than two flow regimes for each type of pedestrian. A subcritical flow always fills the space available. However, a supercritical flow may either fill the space available or be self-confining for each type of pedestrian, depending on the boundary location. Although, the equations governing these flows are simultaneous, time-dependent, non-linear, partial differential equations, remarkably they may be made conformally mappable. The solution of these equations becomes trivial in many situations. Free streamline calculations, utilizing this property, reveal both upstream and downstream separation of the flow of pedestrians around an obstacle. Such analysis tells much about the nature of the assumptions used in various models for the flow of pedestrians. The present theory is designed for the development of general techniques to understand the motion of large crowds. However, it is also useful as a predictive tool. The behavior predicted by these equations of motion is compared with aerial observations for the Jamarat Bridge near Mecca, Saudi Arabia. It is shown that, for this important case, pedestrians, that is pilgrims, aim at achieving each immediate goal in minimum time rather than achieving all goals in overall minimum time. Typical of many examples, this case illustrated the strong dependence of path on the psychological state of the pedestrians involved. It is proposed that the flow of pedestrians over the Jamarat Bridge be improved by appropriate barrier placement, that force an effective global view of the goals.},
keyword={\textit{Keywords: }\textbf{No keywords.}}
}

@article{Treuille2006Continuum,
timestamp={2017.07.01},
 author = {Treuille, Adrien and Cooper, Seth and Popovi\'{c}, Zoran},
 title = {Continuum Crowds},
 journal = {ACM Trans. Graph.},
 issue_date = {July 2006},
 volume = {25},
 number = {3},
 month = jul,
 year = {2006},
 issn = {0730-0301},
 pages = {1160--1168},
 numpages = {9},
 url2 = {http://doi.acm.org/10.1145/1141911.1142008},
 doi = {10.1145/1141911.1142008},
 acmid = {1142008},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {crowds, human simulation, motion planning},
}

@article{Duives2013State,
timestamp={2017.07.01},
title = {State-of-the-art crowd motion simulation models},
journal = {Transportation Research Part C: Emerging Technologies},
volume = {37},
number = {},
pages = {193 - 209},
year = {2013},
noteD = {},
issn = {0968-090X},
doi = {http://dx.doi.org/10.1016/j.trc.2013.02.005},
url2 = {http://www.sciencedirect.com/science/article/pii/S0968090X13000351},
author = {Dorine C. Duives and Winnie Daamen and Serge P. Hoogendoorn},
keywords = {Pedestrian},
keywords = {Crowd phenomena},
keywords = {Pedestrian simulation models},
keywords = {Comparison},
keywords = {Assessment},
keywords = {Self-organization},
abstract = {Currently, pedestrian simulation models are used to predict where, when and why hazardous high density crowd movements arise. However, it is questionable whether models developed for low density situations can be used to simulate high density crowd movements. The objective of this paper is to assess the existent pedestrian simulation models with respect to known crowd phenomena in order to ascertain whether these models can indeed be used for the simulation of high density crowds and to indicate any gaps in the field of pedestrian simulation modeling research. This paper provides a broad, but not exhaustive overview of the crowd motion simulation models of the last decades. It is argued that any model used for crowd simulation should be able to simulate most of the phenomena indicated in this paper. In the paper cellular automata, social force models, velocity-based models, continuum models, hybrid models, behavioral models and network models are discussed. The comparison shows that the models can roughly be divided into slow but highly precise microscopic modeling attempts and very fast but behaviorally questionable macroscopic modeling attempts. Both sets of models have their use, which is highly dependent on the application the model has originally been developed for. Yet, for practical applications, that need both precision and speed, the current pedestrian simulation models are inadequate.}
}

@article{Hoogendoorn2015Continuum,
timestamp={2017.07.01},
title = {Continuum theory for pedestrian traffic flow: Local route choice modelling and its implications},
journal = {Transportation Research Part C: Emerging Technologies},
volume = {59},
number = {},
pages = {183 - 197},
year = {2015},
noteD = {Special Issue on International Symposium on Transportation and Traffic Theory},
issn = {0968-090X},
doi = {http://dx.doi.org/10.1016/j.trc.2015.05.003},
url2 = {http://www.sciencedirect.com/science/article/pii/S0968090X15001746},
author = {Serge P. Hoogendoorn and Femke van Wageningen-Kessels and Winnie Daamen and Dorine C. Duives and Majid Sarvi},
keywords = {Continuum flow modelling},
keywords = {Local route choice},
keywords = {Hybrid modelling},
abstract = {This contribution puts forward a novel multi-class continuum model that captures some of the key dynamic features of pedestrian flows. It considers route choice behaviour on both the strategic (pre-trip) and tactical (en-route) level. To achieve this, we put forward a class-specific equilibrium direction relation of the pedestrians, which is governed by two parts: one part describing the global route choice, which is pre-determined based on the expectations of the pedestrians, and one part describing the local route choice, which is a density-gradient dependent term that reflects local adaptations based on prevailing flow conditions. Including the local route choice term in the multi-class model causes first of all dispersion of the flow: pedestrians will move away from high density areas in order to reduce their overall walking costs. Second of all, for the crossing flow and bi-directional flow cases, local route choice causes well known self-organised patterns to emerge (i.e. diagonal stripes and bi-directional lanes). We study under which demand conditions self-organisation occurs and fails, as well as what the impact is of the choices of the different model parameters. In particular, the differences in the weights reflecting the impact of the own and the other classes appear to have a very strong impact on the self-organisation process.}
}

@article{Yildirimoglu2015Equilibrium,
timestamp={2017.07.01},
title = {Equilibrium analysis and route guidance in large-scale networks with MFD dynamics},
journal = {Transportation Research Part C: Emerging Technologies},
volume = {59},
number = {},
pages = {404 - 420},
year = {2015},
noteD = {Special Issue on International Symposium on Transportation and Traffic Theory},
issn = {0968-090X},
doi = {http://dx.doi.org/10.1016/j.trc.2015.05.009},
url2 = {http://www.sciencedirect.com/science/article/pii/S0968090X15001813},
author = {Mehmet Yildirimoglu and Mohsen Ramezani and Nikolas Geroliminis},
keywords = {Macroscopic fundamental diagram},
keywords = {Route guidance},
keywords = {System optimum},
keywords = {User equilibrium},
abstract = {Recent studies have demonstrated that Macroscopic Fundamental Diagram (MFD), which provides an aggregated model of urban traffic dynamics linking network production and density, offers a new generation of real-time traffic management strategies to improve the network performance. However, the effect of route choice behavior on MFD modeling in case of heterogeneous urban networks is still unexplored. The paper advances in this direction by firstly extending two MFD-based traffic models with different granularity of vehicle accumulation state and route choice behavior aggregation. This configuration enables us to address limited traffic state observability and to scrutinize implications of drivers’ route choice in MFD modeling. We consider a city that is partitioned in a small number of large-size regions (aggregated model) where each region consists of medium-size sub-regions (more detailed model) exhibiting a well-defined MFD. This paper proposes a route guidance advisory control system based on the aggregated model as a large-scale traffic management strategy that utilizes aggregated traffic states while sub-regional information is partially known. In addition, we investigate the effect of equilibrium conditions (i.e. user equilibrium and system optimum) on the overall network performance, in particular MFD functions.}
}

@article{Jiang2012Numerical,
timestamp={2017.07.01},
title = {Numerical simulation of a continuum model for bi-directional pedestrian flow},
journal = {Applied Mathematics and Computation},
volume = {218},
number = {10},
pages = {6135 - 6143},
year = {2012},
noteD = {},
issn = {0096-3003},
doi = {http://dx.doi.org/10.1016/j.amc.2011.11.099},
url2 = {http://www.sciencedirect.com/science/article/pii/S0096300311014457},
author = {Yanqun Jiang and S.C. Wong and Peng Zhang and Ruxun Liu and Yali Duan and Keechoo Choi},
keywords = {Pedestrian counterflow},
keywords = {Continuum model},
keywords = {Reactive dynamic user equilibrium},
keywords = {Eikonal-type equation},
keywords = {Finite volume scheme},
keywords = {Fast sweeping method},
abstract = {An algorithm for an extended reactive dynamic user equilibrium model of pedestrian counterflow as a continuum is developed. It is based on a cell-centered high-resolution finite volume scheme with a fast sweeping method for an Eikonal-type equation on an orthogonal grid. A high-order total variation diminishing Runge–Kutta method is adopted for the time integration of semi-discrete equations. The numerical results demonstrate the rationality of the model and efficiency of the algorithm. Some crowd pedestrian flow phenomena, such as dynamic lane formation in bi-directional flow, are observed which are helpful for a global comprehension of pedestrian dynamics. Also, the model can be utilized with different potential applications.}
}

@article{Hanseler2014Macroscopic,
timestamp={2017.07.01},
title = {A macroscopic loading model for time-varying pedestrian flows in public walking areas},
journal = {Transportation Research Part B: Methodological},
volume = {69},
number = {},
pages = {60 - 80},
year = {2014},
noteD = {},
issn = {0191-2615},
doi = {http://dx.doi.org/10.1016/j.trb.2014.08.003},
url2 = {http://www.sciencedirect.com/science/article/pii/S0191261514001386},
author = {Flurin S. Hanseler and Michel Bierlaire and Bilal Farooq and Thomas Muhlematter},
keywords = {Pedestrian flows},
keywords = {Dynamic network loading},
keywords = {Cell transmission model},
keywords = {Macroscopic model},
keywords = {En-route path choice},
keywords = {Calibration},
abstract = {A macroscopic loading model applicable to time-dependent and congested pedestrian flows in public walking areas is proposed. Building on the continuum theory of pedestrian flows and the cell transmission model for car traffic, an isotropic framework is developed that can describe the simultaneous and potentially conflicting propagation of multiple pedestrian groups. The model is formulated at the aggregate level and thus computationally cheap, which is advantageous for studying large-scale problems. A detailed analysis of several basic flow patterns including counter- and cross flows, as well as two generic scenarios involving a corner- and a bottleneck flow is carried out. Various behavioral patterns ranging from disciplined queueing to impatient jostling can be realistically reproduced. Following a systematic model calibration, two case studies involving a Swiss railway station and a Dutch bottleneck flow experiment are presented. A comparison with the social force model and pedestrian tracking data shows a good performance of the proposed model with respect to predictions of travel time and density.}
}

@article{Jiang2009Reactive,
timestamp={2017.07.01},
title = {A reactive dynamic continuum user equilibrium model for bi-directional pedestrian flows},
journal = {Acta Mathematica Scientia},
volume = {29},
number = {6},
pages = {1541 - 1555},
year = {2009},
noteD = {},
issn = {0252-9602},
doi = {http://dx.doi.org/10.1016/S0252-9602(10)60002-1},
url2 = {http://www.sciencedirect.com/science/article/pii/S0252960210600021},
author = {Yanqun Jiang and Tao Xiong and S.C. Wong and Chi-Wang Shu and Mengping Zhang and Peng Zhang and William H.K. Lam},
keywords = {pedestrian flows},
keywords = {conservation law},
keywords = {Eikonal-type equation},
keywords = {density-velocity relationship},
keywords = {finite volume method},
keywords = {fast marching method},
keywords = {unstructured grids},
keywords = {76M12},
abstract = {In this paper, a reactive dynamic user equilibrium model is extended to simulate two groups of pedestrians traveling on crossing paths in a continuous walking facility. Each group makes path choices to minimize the travel cost to its destination in a reactive manner based on instantaneous information. The model consists of a conservation law equation coupled with an Eikonal-type equation for each group. The velocity-density relationship of pedestrian movement is obtained via an experimental method. The model is solved using a finite volume method for the conservation law equation and a fast-marching method for the Eikonal-type equation on unstructured grids. The numerical results verify the rationality of the model and the validity of the numerical method. Based on this continuum model, a number of results, e.g., the formation of strips or moving clusters composed of pedestrians walking to the same destination, are also observed.}
}

@article{Jiang2010Higher,
timestamp={2017.07.01},
title = {A higher-order macroscopic model for pedestrian flows},
journal = {Physica A: Statistical Mechanics and its Applications},
volume = {389},
number = {21},
pages = {4623 - 4635},
year = {2010},
noteD = {},
issn = {0378-4371},
doi = {http://dx.doi.org/10.1016/j.physa.2010.05.003},
url2 = {http://www.sciencedirect.com/science/article/pii/S0378437110003808},
author = {Y. Q. Jiang and Peng Zhang and S.C. Wong and Ru-xun Liu},
keywords = {Pedestrian crowd dynamics},
keywords = {Path choice},
keywords = {Linear stability analysis},
keywords = {Traffic instability},
keywords = {Unstructured meshes},
keywords = {Obstruction},
abstract = {This paper develops a higher-order macroscopic model of pedestrian crowd dynamics derived from fluid dynamics that consists of two-dimensional Euler equations with relaxation. The desired directional motion of pedestrians is determined by an Eikonal-type equation, which describes a problem that minimizes the instantaneous total walking cost from origin to destination. A linear stability analysis of the model demonstrates its ability to describe traffic instability in crowd flows. The algorithm to solve the macroscopic model is composed of a splitting technique introduced to treat the relaxation terms, a second-order positivity-preserving central-upwind scheme for hyperbolic conservation laws, and a fast-sweeping method for the Eikonal-type equation on unstructured meshes. To test the applicability of the model, we study a challenging pedestrian crowd flow problem of the presence of an obstruction in a two-dimensional continuous walking facility. The numerical results indicate the rationality of the model and the effectiveness of the computational algorithm in predicting the flux or density distribution and the macroscopic behavior of the pedestrian crowd flow. The simulation results are compared with those obtained by the two-dimensional Lighthill–Whitham–Richards pedestrian flow model with various model parameters, which further shows that the macroscopic model is able to correctly describe complex phenomena such as “stop-and-go waves” observed in empirical pedestrian flows.}
}

@article{Hanseler2017Dynamic,
timestamp={2017.07.01},
title = {A dynamic network loading model for anisotropic and congested pedestrian flows },
journal = {Transportation Research Part B: Methodological },
volume = {95},
number = {},
pages = {149 - 168},
year = {2017},
noteD = {},
issn = {0191-2615},
doi = {https://doi.org/10.1016/j.trb.2016.10.017},
url2 = {http://www.sciencedirect.com/science/article/pii/S0191261515301442},
author = {Flurin S. Hanseler and William H.K. Lam and Michel Bierlaire and Gael Lederrey and Marija Nikolic},
keywords = {Pedestrian flow},
keywords = {Network loading},
keywords = {Macroscopic model},
keywords = {Pedestrian fundamental diagram},
keywords = {Anisotropy},
keywords = {Calibration },
abstract = {Abstract A macroscopic loading model for multi-directional, time-varying and congested pedestrian flows is proposed. Walkable space is represented by a network of streams that are each associated with an area in which they interact. To describe this interaction, a stream-based pedestrian fundamental diagram is used that relates density and walking speed in multi-directional flow. The proposed model is applied to two different case studies. The explicit modeling of anisotropy in walking speed is shown to significantly improve the ability of the model to reproduce empirically observed walking time distributions. Moreover, the obtained model parametrization is in excellent agreement with the literature. }
}

@article{Laval2017Minimal,
timestamp={2017.07.01},

title = "Minimal parameter formulations of the dynamic user equilibrium using macroscopic urban models: Freeway vs city streets revisited",
journal = "Transportation Research Part B: Methodological",
year = "2017",
issn = "0191-2615",
doi = "https://doi.org/10.1016/j.trb.2017.08.027",
url2 = "http://www.sciencedirect.com/science/article/pii/S0191261517307464",
author = "Jorge A. Laval and Ludovic Leclercq and Nicolas Chiabaut",
keywords = "Dynamic traffic assignment, Macroscopic fundamental diagram",
abstract = "This paper investigates the dynamic user equilibrium (DUE) on a single origin-destination pair with two alternative routes, a freeway with a fixed capacity and the surrounding city-streets network, modeled with a network macroscopic fundamental diagram (NMFD). We find using suitable transformations that only a single network parameter is required to characterize the DUE solution, the freeway to NMFD capacity ratio. We also show that the stability and convergence properties of this system are captured by the constant demand case, which corresponds to an autonomous dynamical system that admits analytical solutions. This solution is characterized by two critical accumulation values that determine if the steady state is in free-flow or gridlock, depending on the initial accumulation. Additionally, we also propose a continuum approximation to account for the spatial evolution of congestion, by including variable trip length and variable NMFD coverage area in the model. It is found that gridlock cannot happen and that the steady-state solution is independent of surface network parameters. These parameters do affect the rate of convergence to the steady-state solution, but convergence rates appear virtually identical when time is expressed in units of the NMFD free-flow travel time."
}
@article{Algadhi1991Simulation,
timestamp={2017.07.01},
  title={Simulation of crowd behavior and movement: fundamental relations and application},
  author={AlGadhi, Saad AH and Mahmassani, H},
  journal={Transportation Research Record},
  volume={1320},
  number={1320},
  pages={260--268},
  year={1991}
}

@article{Xia2009Dynamic,
timestamp={2017.07.01},
  title = {Dynamic continuum pedestrian flow model with memory effect},
  author = {Xia, Yinhua and Wong, S. C. and Shu, Chi-Wang},
  journal = {Phys. Rev. E},
  volume = {79},
  issue = {6},
  pages = {066113},
  numpages = {8},
  year = {2009},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.79.066113},
  url2 = {https://link.aps.org/doi/10.1103/PhysRevE.79.066113}
}







@article{Boyce1995Solving,
timestamp={2017.07.10},
author = {David E. Boyce and Bin Ran and Larry J. Leblanc},
title = {Solving an Instantaneous Dynamic User-Optimal Route Choice Model},
journal = {Transportation Science},
volume = {29},
number = {2},
pages = {128-142},
year = {1995},
doi = {10.1287/trsc.29.2.128},
url2 = {https://doi.org/10.1287/trsc.29.2.128},
abstract = { Dynamic models of the behavior of automobile drivers in choosing routes through urban transportation networks are required for the design and operation of intelligent transportation systems generally, and traveler information systems in particular. In this paper, drivers' route choice behavior based on current, or instantaneous, information on network conditions is described using an optimal control theory formulation. The time-dependent origin-destination vehicle trip pattern is assumed to be known. The instantaneous dynamic user-optimal route choice problem is to allocate vehicle flows to the current minimal-cost routes, defined as the routes that minimize the route travel cost between each decision node (any node on the route including the origin) and the destination node based on the currently prevailing travel times. The continuous time formulation of the problem is transformed into a discrete time nonlinear programming (NLP) formulation. Each of a sequence of NLPs is then solved by an algorithm based on the Frank-Wolfe technique. In this sequence, approximate link travel times are updated iteratively in order to represent flow propagation over routes. Computational results from applying the algorithm to two test networks conclude the paper.}
}

@article {Xiong2011High,
timestamp={2017.07.11},
author = {Xiong, Tao and Zhang, Mengping and Shu, Chi-Wang and Wong, S.C. and Zhang, Peng},
title = {High-Order Computational Scheme for a Dynamic Continuum Model for Bi-Directional Pedestrian Flows},
journal = {Computer-Aided Civil and Infrastructure Engineering},
volume = {26},
number = {4},
publisher = {Blackwell Publishing Inc},
issn = {1467-8667},
url2 = {http://dx.doi.org/10.1111/j.1467-8667.2010.00688.x},
doi = {10.1111/j.1467-8667.2010.00688.x},
pages = {298--310},
year = {2011},
abstract = {Abstract: In this article, we present a high-order weighted essentially non-oscillatory (WENO) scheme, coupled with a high-order fast sweeping method, for solving a dynamic continuum model for bi-directional pedestrian flows. We first review the dynamic continuum model for bi-directional pedestrian flows. This model is composed of a coupled system of a conservation law and an Eikonal equation. Then we present the first-order Lax–Friedrichs difference scheme with first-order Euler forward time discretization, the third-order WENO scheme with third-order total variation diminishing (TVD) Runge–Kutta time discretization, and the fast sweeping method, and demonstrate how to apply them to the model under study. We present a comparison of the numerical results of the model from the first-order and high-order methods, and conclude that the high-order method is more efficient than the first-order one, and they both converge to the same solution of the physical model.},
}


@article{Lin2017Predictive,
timestamp={2017.07.13},
author = {Z.Y. Lin and S.C. Wong and P. Zhang and Y.Q. Jiang and K. Choi and Y.C. Du},
title = {A predictive continuum dynamic user-optimal model for a polycentric urban city},
journal = {Transportmetrica B: Transport Dynamics},
volume = {5},
number = {3},
pages = {233-252},
year = {2017},
doi = {10.1080/21680566.2016.1163297},

url2 = { 
        http://dx.doi.org/10.1080/21680566.2016.1163297
    
},
eprint = { 
        http://dx.doi.org/10.1080/21680566.2016.1163297
    
}
,
    abstract = {A predictive continuum dynamic user-optimal model is extended to investigate the traffic equilibrium problem for a polycentric urban city with multiple central business districts (CBDs). The road network within the city is assumed to be dense and can be viewed as a continuum in which travellers can choose their routes in a two-dimensional space. Travellers are assumed to choose their route to minimise the actual total cost to the destination (i.e. the CBD). The model consists of two parts: the conservation law part and the Hamilton–Jacobi part. The finite volume method is used to solve each part on unstructured meshes. Because the two parts are closely interconnected and have different initial times, solving the model can be treated as a fixed-point problem, which is solved using a self-adaptive method of successive averages. Numerical experiments for an urban city with two CBDs are presented to demonstrate the effectiveness of the model and the numerical algorithm. }
}


@article{Huang2009Dynamic,
timestamp={2017.07.18},
author = {L. Huang and Y. Xia and S. C. Wong and C.-W. Shu and M. Zhang and W. H. K. Lam},
title = {Dynamic continuum model for bi-directional pedestrian flows},
journal = {Proceedings of the Institution of Civil Engineers - Engineering and Computational Mechanics},
volume = {162},
number = {2},
pages = {67-75},
year = {2009},
doi = {10.1680/eacm.2009.162.2.67},

url2 = {https://doi.org/10.1680/eacm.2009.162.2.67},
abstract = { The development of a bi-directional pedestrian-flow model based on the reactive dynamic user equilibrium principle and the look-ahead behaviour that induces a viscosity effect on movement patterns is described. The pedestrian density in this model is governed by the conservation law, in which the flow flux is implicitly dependent on the density through the stationary Hamilton-Jacobi equation that is solved using a pseudo time-marching approach. A solution algorithm is proposed and a numerical example is used to demonstrate the effectiveness of the methodology. }
}


@article{Daganzo1994Cell,
timestamp={2017.07.20},
title = "The cell transmission model: A dynamic representation of highway traffic consistent with the hydrodynamic theory",
journal = "Transportation Research Part B: Methodological",
volume = "28",
number = "4",
pages = "269 - 287",
year = "1994",
note = "",
issn = "0191-2615",
doi = "http://dx.doi.org/10.1016/0191-2615(94)90002-7",
url2 = "http://www.sciencedirect.com/science/article/pii/0191261594900027",
author = "Carlos F. Daganzo",
abstract = "This paper presents a simple representation of traffic on a highway with a single entrance and exit. The representation can be used to predict traffic's evolution over time and space, including transient phenomena such as the building, propagation, and dissipation of queues. The easy-to-solve difference equations used to predict traffic's evolution are shown to be the discrete analog of the differential equations arising from a special case of the hydrodynamic model of traffic flow. The proposed method automatically generates appropriate changes in density at locations where the hydrodynamic theory would call for a shockwave; i.e., a jump in density such as those typically seen at the end of every queue. The complex side calculations required by classical methods to keep track of shockwaves are thus eliminated. The paper also shows how the equations can mimic the real-life development of stop-and-go traffic within moving queues."
}

@article{Daganzo1995Cell,
timestamp={2017.07.20},
title = "The cell transmission model, part II: Network traffic",
journal = "Transportation Research Part B: Methodological",
volume = "29",
number = "2",
pages = "79 - 93",
year = "1995",
note = "",
issn = "0191-2615",
doi = "http://dx.doi.org/10.1016/0191-2615(94)00022-R",
url2 = "http://www.sciencedirect.com/science/article/pii/019126159400022R",
author = "Carlos F. Daganzo",
abstract = "This article shows how the evolution of multi-commodity traffic flows over complex networks can be predicted over time, based on a simple macroscopic computer representation of traffic flow that is consistent with the kinematic wave theory under all traffic conditions. The method does not use ad hoc procedures to treat special situations. After a brief review of the basic model for one link, the article describes how three-legged junctions can be modeled. It then introduces a numerical procedure for networks, assuming that a time-varying origin-destination (O-D) table is given and that the proportion of turns at every junction is known. These assumptions are reasonable for numerical analysis of disaster evacuation plans. The results are then extended to the case where, instead of the turning proportions, the best routes to each destination from every junction are known at all times. For technical reasons explained in the text, the procedure is more complicated in this case, requiring more computer memory and more time for execution. The effort is estimated to be about an order of magnitude greater than for the static traffic assignment problem on a network of the same size. The procedure is ideally suited for parallel computing. It is hoped that the results in the article will lead to more realistic models of freeway flow, disaster evacuations and dynamic traffic assignment for the evening commute."
}

@TECHREPORT{Weidmann1992,
timestamp={2017.07.21},
	journal = {Schriftenreihe des IVT},
	volume = {90},
	author = {Weidmann, Ulrich},
	publisher = {IVT, Institut für Verkehrsplanung, Transporttechnik, Strassen- und Eisenbahnbau},
	year = {1992},
	language = {de},
	copyright = {In Copyright - Non-Commercial Use Permitted},
	keywords = {FUSSGÄNGERVERKEHR (VERKEHR UND TRANSPORT); PEDESTRIAN TRAFFIC (TRANSPORTATION AND TRAFFIC)},
	size = {84 S.},
	adress = {Zürich},
	DOI = {10.3929/ethz-a-000687810},
	title = {Transporttechnik der Fussgänger. Transporttechnische Eigenschaften des Fussgängerverkehrs, Literaturauswertung}
}

@article{Dijkstra1959Note,
timestamp={2017.07.23},
  title={A note on two problems in connexion with graphs},
  author={Dijkstra, Edsger W},
  journal={Numerische mathematik},
  volume={1},
  number={1},
  pages={269--271},
  year={1959},
  publisher={Springer}
}


@article{Wong2010Bidirectional,
timestamp={2017.07.23},
author = {S. C. Wong and W. L. Leung and S. H. Chan and William H. K. Lam and Nelson H. C. Yung  and C. Y. Liu and Peng Zhang },
title = {Bidirectional Pedestrian Stream Model with Oblique Intersecting Angle},
journal = {Journal of Transportation Engineering},
volume = {136},
number = {3},
pages = {234-242},
year = {2010},

    abstract = { In this paper, we develop a model of bidirectional pedestrian streams with an oblique intersecting angle that represents the crossing interaction of pedestrians moving in different directions on a walking facility. We formulate the model based on Drake’s model in the traffic flow literature, and calibrate it using results from a set of controlled experiments in which two groups of pedestrians were asked to walk in different directions and cross on designated walkways with different levels of pedestrian flow and different intersecting angles. Their movements were video recorded, and macroscopic quantities such as speed, density, and flow were extracted to calibrate the model of bidirectional pedestrian streams. All of the parameters of the calibrated model are statistically significant at the 0.1\% level. }
}


@article{Chabini1998Discrete,
timestamo={2017.07.24},
author = {Ismail Chabini},
title = {Discrete Dynamic Shortest Path Problems in Transportation Applications: Complexity and Algorithms with Optimal Run Time},
journal = {Transportation Research Record: Journal of the Transportation Research Board},
volume = {1645},
number = {},
pages = {170-175},
year = {1998},
doi = {10.3141/1645-21},

url2 = { 
        https://doi.org/10.3141/1645-21
    
},
eprint = { 
        https://doi.org/10.3141/1645-21
    
}
,
    abstract = { A solution is provided for what appears to be a 30-year-old problem dealing with the discovery of the most efficient algorithms possible to compute all-to-one shortest paths in discrete dynamic networks. This problem lies at the heart of efficient solution approaches to dynamic network models that arise in dynamic transportation systems, such as intelligent transportation systems (ITS) applications. The all-to-one dynamic shortest paths problem and the one-to-all fastest paths problems are studied. Early results are revisited and new properties are established. The complexity of these problems is established, and solution algorithms optimal for run time are developed. A new and simple solution algorithm is proposed for all-to-one, all departure time intervals, shortest paths problems. It is proved, theoretically, that the new solution algorithm has an optimal run time complexity that equals the complexity of the problem. Computer implementations and experimental evaluations of various solution algorithms support the theoretical findings and demonstrate the efficiency of the proposed solution algorithm. The findings should be of major benefit to research and development activities in the field of dynamic management, in particular real-time management, and to control of large-scale ITSs. }
}


@article{Chiu2011Dynamic,
timestamp={2017.07.24},
  title={Dynamic traffic assignment: A primer},
  author={Chiu, Yi-Chang and Bottom, Jon and Mahut, Michael and Paz, Alex and Balakrishna, Ramachandran and Waller, Travis and Hicks, Jim},
  journal={Transportation Research E-Circular},
  number={E-C153},
  year={2011}
}


@article {Xia2008Efficient,
timestamp={2017.07.25},
author = {Xia, Yinhua and Wong, S. C. and Zhang, Mengping and Shu, Chi-Wang and Lam, William H. K.},
title = {An efficient discontinuous Galerkin method on triangular meshes for a pedestrian flow model},
journal = {International Journal for Numerical Methods in Engineering},
volume = {76},
number = {3},
publisher = {John Wiley & Sons, Ltd.},
issn = {1097-0207},
url2 = {http://dx.doi.org/10.1002/nme.2329},
doi = {10.1002/nme.2329},
pages = {337--350},
keywords = {pedestrian flow, continuum modeling, reactive dynamic user equilibrium, discontinuous Galerkin method, fast sweeping method, triangular mesh, WENO scheme},
year = {2008},
abstract = {In this paper, we develop a discontinuous Galerkin method on triangular meshes to solve the reactive dynamic user equilibrium model for pedestrian flows. The pedestrian density in this model is governed by the conservation law in which the flow flux is implicitly dependent on the density through the Eikonal equation. To solve the Eikonal equation efficiently at each time level, we use the fast sweeping method. Two numerical examples are then used to demonstrate the effectiveness of the algorithm. Copyright © 2008 John Wiley & Sons, Ltd.},
}

@article{Laval2009Graphical,
timestamp={2017.07.27},
  title={Graphical solution and continuum approximation for the single destination dynamic user equilibrium problem},
  author={Laval, Jorge A},
  journal={Transportation Research Part B: Methodological},
  volume={43},
  number={1},
  pages={108--118},
  year={2009},
  publisher={Elsevier}
}

@article{Saumtally2013Dynamical,
timestamp={2017.07.29},
title ="A dynamical two-dimensional traffic model in an anisotropic network",
journal ="Networks and Heterogeneous Media",
volume ="8",
number ="3",
pages ="663-684",
year ="2013",
issn ="1556-1801",
doi ="10.3934/nhm.2013.8.663",
url2 ="http://aimsciences.org/journals/displayArticlesnew.jsp?paperID=9030",
author ="Tibye  Saumtally and Jean Patrick  Lebacque and Habib  Haj-Salem",
keywords ="Traffic network",
keywords ="network supply",
keywords ="users' demand",
keywords ="partial differential equations",
keywords ="dynamical model",
abstract ="Abstract The aim of this paper is to build a dynamical traffic model in a dense urban area. The main contribution of this article is to take into account the four possible directions of traffic flows with flow vectors of dimension $4$ and not $2$ as in fluid mechanic on a plan. Traffic flows are viewed as confrontation results between users demands and a travel supply of the network. The model gathers elements of intersection theory and two-dimensional continuum networks."
}

@article{Sossoe2015Traffic,
timestamp={2017.07.29},
  title={Traffic flow within a two-dimensional continuum anisotropic network},
  author={Sossoe, K. S. and Lebacque, J. P. and Mokrani, A and Haj-Salem, H},
  journal={Transportation Research Procedia},
  volume={10},
  pages={217--225},
  year={2015},
  publisher={Elsevier}
}

@article{Kurganov2001Semidiscrete,
timestamp={2017.07.31},
  title={Semidiscrete central-upwind schemes for hyperbolic conservation laws and Hamilton--Jacobi equations},
  author={Kurganov, Alexander and Noelle, Sebastian and Petrova, Guergana},
  journal={SIAM Journal on Scientific Computing},
  volume={23},
  number={3},
  pages={707--740},
  year={2001},
  publisher={SIAM}
}

@article{Geroliminis2008Existence,
timestamp={2017.07.31},
  title={Existence of urban-scale macroscopic fundamental diagrams: Some experimental findings},
  author={Geroliminis, Nikolas and Daganzo, Carlos F},
  journal={Transportation Research Part B: Methodological},
  volume={42},
  number={9},
  pages={759--770},
  year={2008},
  publisher={Elsevier}
}

@article{Daganzo2007Urban,
  title={Urban gridlock: Macroscopic modeling and mitigation approaches},
  author={Daganzo, Carlos F},
  journal={Transportation Research Part B: Methodological},
  volume={41},
  number={1},
  pages={49--62},
  year={2007},
  publisher={Elsevier}
}

@article{Laval2015Stochastic,
timestamp={2017.07.31},
  title={Stochastic approximations for the macroscopic fundamental diagram of urban networks},
  author={Laval, Jorge A and Castrill{\'o}n, Felipe},
  journal={Transportation Research Part B: Methodological},
  volume={81},
  pages={904--916},
  year={2015},
  publisher={Elsevier}
}

@article{Chiabaut2014Performance,
  title={Performance analysis for different designs of a multimodal urban arterial},
  author={Chiabaut, Nicolas and Xie, Xiaoyan and Leclercq, Ludovic},
  journal={Transportmetrica B: Transport Dynamics},
  volume={2},
  number={3},
  pages={229--245},
  year={2014},
  publisher={Taylor \& Francis}
}

@article{Chiabaut2015Evaluation,
  title={Evaluation of a multimodal urban arterial: The passenger macroscopic fundamental diagram},
  author={Chiabaut, Nicolas},
  journal={Transportation Research Part B: Methodological},
  volume={81},
  pages={410--420},
  year={2015},
  publisher={Elsevier}
}

@article{Fosgerau2015Congestion,
timestamp={2017.08.01},
  title={Congestion in the bathtub},
  author={Fosgerau, Mogens},
  journal={Economics of Transportation},
  volume={4},
  number={4},
  pages={241--255},
  year={2015},
  publisher={Elsevier}
}

@article{Daganzo2008Analytical,
timestamp={2017.08.01},
  title={An analytical approximation for the macroscopic fundamental diagram of urban traffic},
  author={Daganzo, Carlos F and Geroliminis, Nikolas},
  journal={Transportation Research Part B: Methodological},
  volume={42},
  number={9},
  pages={771--781},
  year={2008},
  publisher={Elsevier}
}

@article{Smeed1967Road,
  timestamp={2017.10.23},
  title={The road capacity of city centers},
  author={Smeed, Re J},
  journal={Highway Research Record},
  number={169},
  year={1967}
}

@article{Herman1979Two,
  timestamp={2017.10.23},
  title={A two-fluid approach to town traffic},
  author={Herman, Robert and Prigogine, Ilya},
  journal={Science},
  volume={204},
  number={4389},
  pages={148--151},
  year={1979},
  publisher={American Association for the Advancement of Science}
}

@article{Herman1984Characterizing,
  timestamp={2017.10.23},
  title={Characterizing traffic conditions in urban areas},
  author={Herman, Robert and Ardekani, Siamak},
  journal={Transportation Science},
  volume={18},
  number={2},
  pages={101--140},
  year={1984},
  publisher={INFORMS}
}

@article{Laval2016Symmetries,
timestamp={2017.11.09},
title = "Symmetries in the kinematic wave model and a parameter-free representation of traffic flow",
journal = "Transportation Research Part B: Methodological",
volume = "89",
number = "Supplement C",
pages = "168 - 177",
year = "2016",
issn = "0191-2615",
doi = "https://doi.org/10.1016/j.trb.2016.02.009",
url2 = "http://www.sciencedirect.com/science/article/pii/S0191261515301016",
author = "Jorge A. Laval and Bhargava R. Chilukuri",
keywords = "Traffic flow, Kinematic wave model, Source term"
}

@article{Aghamohammadi2018Dynamic,
title = "Dynamic traffic assignment using the macroscopic fundamental diagram: A Review of vehicular and pedestrian flow models",
journal = "Transportation Research Part B: Methodological.",
year = "2018",
issn = "0191-2615",
note="In Press, Online at: \href{https://doi.org/10.1016/j.trb.2018.10.017}{https://doi.org/10.1016/j.trb.2018.10.017}",
doi2={https://doi.org/10.1016/j.trb.2018.10.017},
url2 = "http://www.sciencedirect.com/science/article/pii/S0191261517311566",
author = "Rafegh Aghamohammadi and Jorge A. Laval",
keywords = "Dynamic traffic assignment, Macroscopic fundamental diagram, Continuum modeling, Multi-reservoir modeling, Pedestrian",
abstract = "Link-level Dynamic Traffic Assignment (DTA) models of large cities may suffer from prohibitive computation times, and calibration/validation can become the major challenge faced in their real-time implementation. The empirical evidence in 2008 in support of the existence of a Macroscopic Fundamental Diagram (MFD) on urban networks led to the formulation of discrete-space DTA models, where the link-level representation of networks replaced by a zone-based representation. In parallel, a large body of DTA models based on Hughes’ pedestrian model have been formulated in continuum space as 2-dimensional conservation laws, where the speed-density relationship has been recently interpreted as a MFD. Unfortunately, today it is not clear whether the continuum-space and discrete-space approaches are consistent with each other, in the sense that a well-defined discrete-space model should correspond to the numerical solution of a continuum model. This paper aims to shed light on this matter by performing a review of the literature in both modeling approaches. We found that (i) the discrete-space DTA models are prone to stalling problem leading to unrealistic gridlocks, (ii) with the exception of Hänseler’s pedestrian models, existing discrete-space models are not guaranteed to be consistent with a continuum formulation, which presents the potential for significant biases between the two approaches although they are trying to answer the same question, (iii) the speed-density relationships used in the continuum-space literature are very simplistic and do not incorporate the effects of network, particularly the effects of intersections, which is the strong suit of the MFD, (iv) the models mostly have been applied to the cases with only one or a few destinations and do not seem to be capable of modeling large-scale networks. We also found that further research is needed to (i) incorporate departure time choice, (ii) improve existing numerical methods, possibly extending recent advances on the one-dimensional kinematic wave (LWR) model, (iii) study the properties of system optimum solutions, (iv) examine the real-time applicability of current continuum-space models compared to traditional DTA methods, and (v) formulate anisotropic models for the interaction of intersecting flows."
}


@article{Carey2004Exit,
timestamp={2017.12.01},
title = "An exit-flow model used in dynamic traffic assignment",
journal = "Computers \& Operations Research",
volume = "31",
number = "10",
pages = "1583 - 1602",
year = "2004",
issn = "0305-0548",
doi = "https://doi.org/10.1016/S0305-0548(03)00109-6",
url2 = "http://www.sciencedirect.com/science/article/pii/S0305054803001096",
author = "Malachy Carey and Mark McCartney",
abstract = "Abstract We consider the behaviour of a link exit-flow model that has been used to model link flows in dynamic traffic assignment (DTA) on networks. In particular, we investigate how the model behaves when time and space (the link length) discretised and the discretisation is varied. We present numerical examples based on various inflow patterns and exit-flow functions and draw conclusions for applications of the model in discrete space and in discrete or continuous time. If inflows are always less than capacity and the link is homogeneous, with no obstructions at the exit, then if the discretisation is refined to the continuous limit the model goes to the solution of the well-known LWR model. However, we observe, somewhat counter intuitively, that the usual continuous-time model does not give as good an approximation to the LWR solution as does the discrete-time model: for a best approximation, the discretisation of space and time should be synchronised. We also investigate the ‘dip’ in outflows, or ‘jamming’ of outflows, that the model displays if inflows are permitted to exceed a capacity limit (as they sometimes do in published applications of the model) and the exit-flow function has a downward sloping part (which has usually been assumed away in DTA applications). In that case, if the number of spatial segments is increased, or the number of time intervals is reduced, then any dip in outflows occurs sooner and is more pronounced, and leads to earlier jamming. In the continuous limit, the jam occurs at the link entrance, preventing inflows in excess of capacity."
}

@article{Carey2012Dynamic,
timestamp={2017.12.01},
title = "Dynamic traffic assignment approximating the kinematic wave model: System optimum, marginal costs, externalities and tolls",
journal = "Transportation Research Part B: Methodological",
volume = "46",
number = "5",
pages = "634 - 648",
year = "2012",
issn = "0191-2615",
doi = "https://doi.org/10.1016/j.trb.2012.01.008",
url2 = "http://www.sciencedirect.com/science/article/pii/S0191261512000094",
author = "Malachy Carey and David Watling",
keywords = "Cell transmission model, System optimum, Dynamic traffic assignment, Marginal costs, Externalities, Optimal tolls",
abstract = "Abstract System marginal costs, externalities and optimal congestion tolls for traffic networks are generally derived from system optimising (SO) traffic assignment models and when they are treated as varying over time they are referred to as dynamic. In dynamic system optimum (DSO) models the link flows and travel times or costs are generally modelled using so-called ‘whole link’ models. Here we instead develop an SO model that more closely reflects traffic flow theory and derive the marginal costs and externalities from that. The most widely accepted traffic flow model appears to be the LWR (Lighthill, Whitham and Richards) model and a tractable discrete implementation or approximation to that is provided by the cell transmission model (CTM) or a finite difference approximation (FDA). These handle spillbacks, traffic controls and moving queues in a way that is consistent with the LWR model and hence with the kinematic wave model and fluid flow model. An SO formulation using the CTM is already available, assuming a single destination and a trapezoidal flow-density function. We extend the formulation to allow more general nonlinear flow density functions and derive and interpret system marginal costs and externalities. We show that if tolls computed from the DSO solution are imposed on users then the DSO solution would also satisfy the criteria for a dynamic user equilibrium (DUE). We extend the analysis to allow for physical or behavioural constraints on the link outflow proportions at merges and inflow proportions at diverges. We also extend the model to elastic demands and establish connections between the present DSO model and earlier DSO models."
}

@article{Friesz1989Dynamic,
timestamp={2017.12.01},
author = {Terry L. Friesz and Javier Luque and Roger L. Tobin and Byung-Wook Wie},
title = {Dynamic Network Traffic Assignment Considered as a Continuous Time Optimal Control Problem},
journal = {Operations Research},
volume = {37},
number = {6},
pages = {893-901},
year = {1989},
doi = {10.1287/opre.37.6.893},

URL2 = { 
        https://doi.org/10.1287/opre.37.6.893
    
},
eprint = { 
        https://doi.org/10.1287/opre.37.6.893
    
}
,
    abstract = { Two continuous time formulations of the dynamic traffic assignment problem are considered, one that corresponds to system optimization and the other to a version of user optimization on a single mode network using optimal control theory. Pontryagin's necessary conditions are analyzed and given economic interpretations that correspond to intuitive notions regarding dynamic system optimized and dynamic user optimized traffic flow patterns. Notably, we offer the first dynamic generalization of Beckmann's equivalent optimization problem for static user optimized traffic assignment in the form of an optimal control problem. The analysis further establishes that a constraint qualification and convexity requirements for the Hamiltonian, which together ensure that the necessary conditions are also sufficient, are satisfied under commonly encountered regularity conditions. }
}



@article{Merchant1978Model,
timestamp={2017.12.01},
author = {Deepak K. Merchant and George L. Nemhauser},
title = {A Model and an Algorithm for the Dynamic Traffic Assignment Problems},
journal = {Transportation Science},
volume = {12},
number = {3},
pages = {183-199},
year = {1978},
doi = {10.1287/trsc.12.3.183},

URL2 = { 
        https://doi.org/10.1287/trsc.12.3.183
    
},
eprint = { 
        https://doi.org/10.1287/trsc.12.3.183
    
}
,
    abstract = { A discrete time model is presented for dynamic traffice assignment with a single destination. Congestion is treated explicitly in the flow equations. The model is a nonlinear and nonconvex mathematical programming problem. A piecewise linear version of the model, with additional assumptions on the objective function, can be solved for a global optimum using a one-pass simplex algorithm—branch-and-bound is not required. The piecewise linear program has a staircase structure and can be solved by decomposition techniques or compactification methods for sparse matrices. }
}

@article{Lighthill1955Kinematic,
timestamp={2017.12.06},
 author = {M. J. Lighthill and G. B. Whitham},
 journal = {Proceedings of the Royal Society of London. Series A, Mathematical and Physical Sciences},
 number = {1178},
 pages = {317-345},
 publisher = {The Royal Society},
 title = {On Kinematic Waves. II. A Theory of Traffic Flow on Long Crowded Roads},
 volume = {229},
 year = {1955},
 ISSN = {00804630},
 URL2 = {http://www.jstor.org/stable/99769},
 abstract = {This paper uses the method of kinematic waves, developed in part I, but may be read independently. A functional relationship between flow and concentration for traffic on crowded arterial roads has been postulated for some time, and has experimental backing (§2). From this a theory of the propagation of changes in traffic distribution along these roads may be deduced (§§2, 3). The theory is applied (§4) to the problem of estimating how a 'hump', or region of increased concentration, will move along a crowded main road. It is suggested that it will move slightly slower than the mean vehicle speed, and that vehicles passing through it will have to reduce speed rather suddenly (at a 'shock wave') on entering it, but can increase speed again only very gradually as they leave it. The hump gradually spreads out along the road, and the time scale of this process is estimated. The behaviour of such a hump on entering a bottleneck, which is too narrow to admit the increased flow, is studied (§5), and methods are obtained for estimating the extent and duration of the resulting hold-up. The theory is applicable principally to traffic behaviour over a long stretch of road, but the paper concludes (§6) with a discussion of its relevance to problems of flow near junctions, including a discussion of the starting flow at a controlled junction. In the introductory sections 1 and 2, we have included some elementary material on the quantitative study of traffic flow for the benefit of scientific readers unfamiliar with the subject.}
}

@article{richards1956shock,
  title={Shock waves on the highway},
  author={Richards, Paul I},
  journal={Operations research},
  volume={4},
  number={1},
  pages={42--51},
  year={1956},
  publisher={INFORMS}
}

% different state representation, action space and reward function, different simulator for modeling the environment
% the algorithm they adopted



% Existing studies using DRL for large-scale traffic control can be generally classified into two categories.i.e. decetralized control with multi-agents and a centralized control method with advanced DRL algorithms.

% i) the decentralized method takes advantage of multiple agents and designs efficient communication and coordination among them to address the limitation of partial observation of the environment for individual agents. It generally requires to decompose the large network into small regions or individual intersections, conduct RL for each task, and train their policy with communication and coordination \cite{khamis2014adaptive,wei2019colight,tan2019cooperative,gong2019decentralized}. It is worth noting that different observations from the environment have been used as communication information between agents, such as neighbouring intersections, downstream intersections or upstream intersections. How to incorporate those external information and trade-off the balance between their own state and local rewards remain as an open research question. 


% ii) the other pipeline of the work enhances the algorithm and extends them to the high-dimensional continuous control problems, such as devising novel algorithms with e.g. advantage actor-critic, memory replay and target network. Semantic works can be found in \cite{lillicrap2015continuous,mnih2015human} and the applications in large-scale traffic control are seen in \cite{genders2016using,li2016traffic,chu2016large}. 

% SUMO allows the RL intersections, a.k.a. the intersection signals to interact and learn from the environment.  An extended study \cite{wu2017framework} developed a Customized Interface for SUMO, TraCI, and RLLab library (\textbf{CISTAR}), a framework for reinforcement learning and control experiments for traffic microsimulation, it integrates the traffic simulator SUMO with a standard deep reinforcement learning library RLLab and support high frequency simulation and more flexibility in controllers.


We argue that instead of simply improving communication and coordination among multiple agents or enhancing the centralized DRL algorithm, we can tackle the 'curse of dimensionality' in traffic control problems by lending help from the traffic domain knowledge, such as designing simpler state/action representation, more efficient environment (traffic simulator). How to incorporate domain knowledge to constraint the feasible state and actions remains unknown and needs more research attention. 

% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{episodic or continuing?}
% While most of studies adopted algorithms for episodic problems and often terminated after certain peroid of time without an explicit termination condition, we argue that the traffic signal control is instead, a continuing problem.  


%%%%%%%%%%%%%%%%%%%%%%%%% potential explanations by Hao %%%%%%%%%%%%%%%%%%
We conjecture that the deterioration issue under high densities might come from the following aspects: 
\begin{enumerate}
    \item under high densities, the state space, aka the input to our neural network, is almost invariant and such less variance of states will add complexity for the neural network to learn a good policy.
    \item the reward function, aka the throughput, can distinguish good policies from others given low traffic demand, however it is unable to recognize and discriminate good policies under heavy congestion, because any policy seem to yield similar throughput as revealed before. 
    \item the environment CA model assumes only 5 cells for each link with a binary value representing the vehicle occupancy. While it is assumed with maximum simplicity for computational convenience, we admit that such procession of traffic state will certainly lose some detail features, and worse still, in heavy congestion, the state would be almost the same. 
\end{enumerate}


%which is harder to train. The reward signal will be heavily influenced by changes in the demand, rather than by the agent actions, which may corrupt the learning process. If the demand varies slowly, this is likely not to be an issue, however this is not typically the case.
%As for the effect of network congestion levels  on the learned policies, we will show that a policy trained on a particular congestion level, say low  traffic density,  might not perform well under a different level, say high density. The challenge of incorporating different average network densities in the training process is that the reward function, usually throughput,  will change not only due to the agent actions as expected, but also as a result of changes in the density. This will send mixed signals to the learning algorithm and corrupt the solution. 

%Except the state representation, reward and environment dynamics, we suspect that the limitation of REINFORCE algorithm might also be responsible for the failure of policy convergence, if it is not the most critical reason in fact. A critical challenge for REINFORCE algorithm is the high variance of gradient estimator, which is particularly exacerbated in long horizon problems \citep{wu2018variance}. To reduce the variance in gradient estimator, three approaches are often employed: i) only focus on the future cumulative rewards to recognize a good policy ii) add discount factor for future rewards to assign more credit to actions in the immediate near future. iii) use simple baseline to measure the goodness of actions. However, in this study, the traffic control problem as treated as a continual problem due to its non-termination process. Thus no future reward or discount factor can be added. The infinite horizon of continual learning further makes REINFORCE cumbersome. For the converging property, as addressed in \citep{sutton2018reinforcement}, REINFORCE algorithm only guarantees the asymptotic convergence to local optimum. In addition, REINFORCE algorithm is essentially a Monte Carlo method, it needs to estimate the policy goodness based on a batch of trajectory samples, which are not convenient with continual problems.  


%The deterioration under high-density cases reveals some important issues that have not been fully discussed in current DRL research. It turns out the promising outcome of DRL still needs very careful state representation, a good design of reward function and we must have a deep understanding of the environment dynamics such as the impact of traffic demand. Our study also instantiated the issues of REINFORCE algorithm, including its incompatibility with continual problem, the high variance, the instability and limited convergence performance to local optimum. 

%From the perspective of traffic considerations, we suggest if there already exists a good expert policy, maybe DRL is not the best or first choice for us. Even with DRL, we might think about getting rid of the implicit reward functions, and use imitation learning or inverse RL methods to directly mimick the distribution of expert behaviors 88ref (there are plenty of works related to autonomous driving). 

% maybe we can enumerate all the state distribution under different densities, and see how they are distributed.

% I am trying to locate some literature to discuss the issue of 'too similar states'. I suspect too similar states would make the algorithm diverge. 

%

The effect of route choice.

%  The main question is the feasibility region of the MFD that prevents training under congestive conditions; also check that this is not in the literature...

%% The dynamic traffic demand would need a life-long continual learning involving different tasks, which is out of the scope of our study, good references can be seen \citep{}....




%We will see that this definition of reward is superior to the more standard \textit{average flow per lane}, in which case  the average reward  $ \eta (\pi ) $ can be interpreted as the network MFD under policy $\pi$, with the exception that the argument for the average reward is the state vector and that of the MFD is the average density in the network, which are clearly related.


%They found that none of the learning methods is able to cope with high traffic demand, and also claimed that it is due to the agents basically observing same state under heavy congestion. 
%It is worth noting that they adopted a even simpler state representation than ours, in which a link was treated as only one cell, which has only three possible states, i.e. empty, regular and full based on vehicle occupation. In their study, the policy was trained with periodically variant traffic demand, they drew the similar conclusion that there does not exist a universal learned policy which behaves well under different traffic regimes. And they developed the RL algorithm with partial model to predict the varying environment dynamics including the transition probabilities and reward functions. Also note that they adopted different reward functions rather than MFD, but reported the same learning failures, which indicated that the deterioration of policy performance is not related to MFD theory itself, but results from the learning process. 
%Our results indicate that the problem resides on the flow being independent of the policy under congestion.


==> sequel.tex <==
That $w_0\approx4/3$ across all controls and networks is certainly unexpected. Previous theories based on arterial corridors with no turning maintain the symmetry property of the kinematic wave model; e.g., in this case we would have predicted $w_0=u_0$ as given by \eqref{u0}. Using $u_0=w_0\approx4/3$ in \eqref{u0} gives $\lambda\approx 1$, which would normally mean that the average green time produced by the policy equals the mean average between traffic lights $\ell$ (in our scaling). But in our case this means that $\ell$ equals the average \textit{effective} green time, $g'$, defined as the time during the green phase where traffic is actually able to discharge, i.e. the expected green time minus the time the green phase is blocked by downstream traffic. 




Therefore, that an optimal policy produce  $\lambda\approx 1$ is not surprising as it indicates that green times are just long enough  as to not produce spill back.
This highlights the importance of considering segment length when deciding signal timing, a subject rarely mentioned in the signal control literature. 


In the next section we propose a simplified model of urban networks to explain some of these remarks.

\subsection{A Bernouilli model for urban networks}

In this section we present a probabilistic model to approximate the demand MFD under the baseline signal control policies in this paper. As in the one-dimensional kinematic wave model, the demand function represents the flow on a small road segment that would be possible at a given density if downstream bottlenecks are removed; similarly, the supply function gives the maximum flow that the segment can accept. The actual flow turns out to be the minimum of the two. Unlike the kinematic wave model, however, we have seen in \ref{loss of symmetry} that there is a loss of symmetry in the MFD, which implies that demand and supply functions are not symmetric for urban networks. 

Assume that at the initial time $t_0=0$ the number of vehicles in the network is described by a Bernoulli process across all cells in the network, with probability of success $k$, the average density of vehicles in the network. As before, all intersections have 4 approaches, 2 in the NS axis and 2 in the EW axis. Let $N_i^j, i=1,2, j=0,1,\ldots$ be the number of vehicles in each axis wanting to cross a particular intersection during cycle $j$, $i=1$ for NS and $i=2$ for EW. 

We further assume that (i) link lengths are constant and equal to $\ell$, (ii) the green time is long enough to discharge all queued vehicles stored in the approach, even at jam density, i.e. $\lambda=1$ in $g=\ell(1/u+1/w)/\lambda$, and (iii) intersection discharge is not blocked by downstream traffic.

It follows that all vehicles stored in the approach up to the beginning of the green will be able to discharge during that green phase. Therefore, intersection throughput is proportional to $N_i^j$ in our case.
In particular,
the cumulative distribution of $N_i^0,$ namely $F_N^0(n)=\text{Prob}(N_i^0\le n)$, is binomial with parameters $2\ell$ and $k$:
\begin{equation}\label{FN0}
    F_N^0\sim\text{Bin}(2\ell,k)
\end{equation}
The distributions for following cycles, $F_N^j, j=1,2,\ldots$ will depend on the signal control being implemented. For example, under the LQF policy the number of vehicles that will cross during the very first green time in our setup is given by
$\max\{N_1^{0}, N_2^{0}\}$. Since $N_1^{0}, N_2^{0}$ are independent it follows from the theory of extreme value distributions that its CDF is given by $ F_N^0(n)^2$.
Deriving these distributions exactly for continuing cycles quickly becomes intractable, unfortunately, mainly because there are too many combinations to consider regarding which axes gets the green light of surrounding intersections. 
But for spatially homogeneous networks with random vehicle routing, all intersections have to be probabilistically identical. This means that the input and output off all intersections should follow the same distribution, which unfortunately is not easy to obtain. % CDF $ F_N^0(n)^2$ under LQF.  
As an approximation, we propose: 
\begin{subequations}\label{Nij}
\begin{empheq}[left={N_i^{j+1}=\empheqlbrace\,}]{align}
    \max\{N_1^{j},\ N_2^{j}\} & \qquad \text{(LQF)} \label{Nija}\\
    \min\{N_1^{j},\ N_2^{j}\} & \qquad \text{(SQF)} \label{Nijb}\\
    N_1^{j} \qquad \qquad & \qquad \text{(Random)} \label{Nijc}
    \end{empheq}
\end{subequations}
This approximation reflects that the output of a given intersection, e.g. $\max\{N_1^{j}, N_2^{j}\}$  for LQF and $\min\{N_1^{j}, N_2^{j}\}$ for SQF,
corresponds to input for downstream intersections for the following cycle, i.e, to the number of vehicles waiting to cross the two downstream intersections during the following cycle. Notice that the random policy does not change the distribution of the output. 
To obtain the distribution under LQF (resp. SQF), we unwind the RHS of \eqref{Nija}  (resp. \eqref{Nijb}) to obtain the maximum (resp. minimum) of $2j$ i.i.d. random variables distributed according to $F_N^0(n)$. Therefore,
\begin{equation}\label{FNj}
    F_N^j(n) = \begin{cases}
 F_N^0(n)^{2j} & \text{(LQF)} \\
 1-(1-F_N^0(n))^{2j} & \text{(SQF)} \\
 F_N^0(n) & \text{(Random)} \\
 \end{cases}
\end{equation}


\cite{dag11}

The flow in axis $i$ through the intersection in our case is simply proportional to $N_i^j$, as mentioned at the outset. It  is given by the fundamental traffic flow relationship, i.e. the product of density, $\fracjl{N_i^j}{2 \ell}$, and free-flow speed  $u$. To compare with the MFD's obtained by simulation, we compute the average flow per lane through the intersection, $Q_i^j$:
\begin{equation}\label{Qi}
    Q_i^j = \frac{1}{4}\cdot\frac{u N_i^j}{2 \ell},
\end{equation}
The factor 4 comes in because \eqref{Nij} gives the flow of the two opposing  approaches combined and only during the green phase, which is half of the cycle time in our case.
It follows that the CDF of the flow is
\begin{equation}\label{FQi}
    F_{Q}^j(q)=F_N^j(8\ell q/u)
\end{equation}


It turns out that this distribution exhibits strikingly similar behavior to the simulation results for all 3 strategies. This is shown in
Fig.~\ref{fFQ}, where the shaded areas represent the 90\%-probability interval (between the 5th and the 95th percentile) of the flow distribution \eqref{FQi} for the three baseline policies and for several values of $j$. It can be seen that for $j\ge 10$ the demand MFD produced by the control strategies accord well with simulation results in Fig.~\ref{MFDs}.

%These lower bounds are \textit{optimistic} compared to our CA traffic model because this binomial approximation incorporates either lost times or minimum green, and thus the traffic model percentiles should be lower than the approximation.

For the upper bounds, the method of cuts provides the answer, and the reader is referred to \citep{daganzo2008analytical, Laval2015Stochastic} for the details. 
Given this upper bound, it becomes clear that the congested states beyond the intersection point ``A'' in  Fig.~\ref{mfd} obey very different rules compared to congestion near capacity. In this extreme congestion state the control has absolutely no influence on network flow, which is deterministic in which explains the failure of DRL methods to learn (because there is nothing to learn!). In moderate congestion closer to the critical density the flow is stochastic and the lower bound starts activating, causing the distance between upper and lower bounds to decrease with density, which might explain the learning difficulties in this traffic state.  Moderate free-flow is similar, except that the lower bound remains at zero flow. Finally, extreme free-flow is different than extreme congestion because in the former the lower bound is zero.

\begin{figure}[tb]
\centering
\includegraphics[width=.495\textwidth]{qunt.png}
%\includegraphics[width=.495\textwidth]{quntUpper.png}
\caption{Percentiles for the minimum %(left) and maximum (right) 
of two independent binomial random variables with parameters $2n$ and $k$.}
\label{quantic}
\end{figure}

The above paragraph suggests that at any given density the distance between the upper bound in congestion and the lower bound is a measure of the potential for DRL methods to learn. This ``learning potential'' is maximum in free-flow and starts shrinking %at the critical density 
until disappearing at point ``A'' in  Fig.~\ref{mfd}. But in practice this learning potential might be much narrower than shown in the figure, which explains why learning difficulties start near the critical density. To see this, consider the median outflow in Fig.~\ref{quantic} (left), which  indicates that most of the time a bad policy will produce remarkably high flows; e.g. for $k=0.5$ the median outflow is around 0.2.
But this high outflow will be above the upper bounds in Fig.~\ref{mfd}. This means that most of the time the throughput of an intersection is dictated by the infrastructure (the upper bounds) rather than the policy.
This is the simplest explanation consistent with the results in this paper, but research is needed to understand how to use it for learning under congestive conditions.




==> table.tex <==
\begin{landscape}
% [insert table here that will be displayed horizontally]
\begin{center}
\begin{tabular}{|p{1.5cm}||p{2.5cm}|p{3cm}|p{4cm}|p{1.5cm}|p{5cm}|}
%  \multicolumn{5}{|c|}{Related work} \\
 \hline
 Studies & RL models & Traffic Simulator & Domain knowledge & Epis/cont & Performance measurement\\ 
 \hline
 \cite{chu2015traffic} & Approximation Q-learning  & a macroscopic network model & integrating MFD theory & Epis & Convergence \\
 \cite{aslani2018traffic} & multiple DRLs  & AIMSUM  & testing algorithm robustness with system disturbances & Epis & Comparing average travel time under different algorithms as well as an optimized fixed time controller \\
 \cite{tan2019cooperative} & hierarchical DRL & SUMO & manual regional partition & Epis & Comparing algorithm with traffic performance measures \\
 \cite{chu2019multi} & Multi-agent A2C  & SUMO &  N.A. & Epis & queue length and network vehicle accumulation \\
 \cite{ge2019cooperative} & Q-value transfer & CA-similar model  & the optimal Q-values of the neighbor agents are transferred & Epis & comparing traffic performance cross algorithms \\
 \hline
\end{tabular}
\end{center}
\end{landscape}

